Tutorial on the Quantikz Package

This tutorial introduces (and provides, via the document source) the Quantikz LaTeX package for typesetting quantum circuit diagrams. This takes advantage of tikz to give greater control over the circuit options. Those familiar with the excellent QCircuit package will recognise much of the notation, although it has evolved a bit (hopefully simplified!).

==> tikzlibraryquantikz2.code.tex <==
%This is the quantikz library for typesetting quantum circuits using LaTeX/Tikz. version 1.0.3
% Written by Alastair Kay, 2018. Published under a CC-BY-4.0 licence
% Please email me (alastair.kay@rhul.ac.uk) with any bug reports or feature requests.
% If you find this library useful, please cite its usage in your work, using arXiv:1809.03842.
% Usage is at your own risk.

%version 1.1.5
%aim is to produce an extra file that contains useful alt text for a circuit.
%\quantikzAltText{} switches on the output of alt text to a file specified in the required argument. From here on, alt text for quantum circuits is automatically generated and output.
%\quantikzEndAltText put at the end of the documents. Just closes the output file.
%\figAltText{} best placed inside caption of a figure. It records alt text for the figure. Can also be used for inline images.
%version 1.1.0
% lots of background work to improve key handling.
% reduces risk of macros colliding with those of other packages
% Vastly reduced the number of "\expandafter"s. Hopefully improves performance
%version 1.0.2
% added meterout command
% classical gap has been separated into two different distances, for horizontal and vertical.
% future: vertical distance could be separated into classical wire gap and bundle gap. Would need a bit of recoding on the wire.
% added cbend command that does a 90 degree classical wire curve.
% gate (and many other, most noticably inputD) commands didn't work in the very first cell. Should now be fixed.
% completely removed the possibility of using tikzcd environment directly. This improves compatibility with other packages that want to use tikzcd. See e.g. https://tex.stackexchange.com/questions/689265/how-do-i-use-both-quantikz-and-zx-calculus-packages
% fixed horizontal size of phantom gates.
%fixed bug I then introduced that prevented slice all from working
%slices now inherit the global set options from slice style and slice label style, but local options still take priority.
%fixed a bug where cell widths didn't reset if cell not declared by &
%version 1.0.1
% the lstick/midstick/rstick commands now correctly resize braces if you're using classical wires based on wire types at the *end* of each wire (so rstick more likely to look good than lstick/midstick!.
% fixed incompatibility if physics2 package (turned out we both used the same variable name somewhere)
%version 1.0.0
%major new revision with massive under-the-hood changes in how wires work.
%aiming to reduce technical debt in the code as well.
%use the \wire commands for all your wire needs
%fix wire types using wire types={} key, and function setwiretype{}
%check your circuits for places where you assumed there would be no wire.
%some minor changes in optional parameters (e.g. \meter). In practice, these are rarely used, and unlikely to be an issue.
%should always use quantikz and not tikzcd environment

%\ProvidesPackage{quantikz}[2023/05/24 typeset quantum circuit diagrams]

% Package(s) to include
\RequirePackage{xargs,ifthen,xstring,etoolbox,mathtools,pgfmath}
\RequirePackage{refcount}
\RequirePackage{environ} %in an attempt to help with compatibility with the external library of tikz.
%\RequirePackage{tikz}
\usetikzlibrary{cd,decorations.pathreplacing,calc,positioning,fit,shapes.symbols,decorations.pathmorphing,shapes.misc,decorations.markings,math}
\pgfdeclarelayer{background}
\pgfdeclarelayer{quantback}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%create the new quantikz environment
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%I need this to facilitate the external library
%solution taken from https://tex.stackexchange.com/questions/171931/are-the-tikz-libraries-cd-and-external-incompatible-with-one-another
%this does a global redefinition of the &. This is not good as it will lead to incompatibilities with other packages.
%there seems to be a solution https://tex.stackexchange.com/a/633066/148934
%another option, more similar to the original: https://tex.stackexchange.com/a/619983/148934

%full solution suggested here https://tex.stackexchange.com/a/682872/148934
\ExplSyntaxOn
\NewDocumentEnvironment{quantikz}{O{}+b}{%
\gdef\toslice@qtkz{0}\def\vert@qtkz{0}%
\quantikz@startAltText
  \begin{tikzpicture}[/tikz/commutative~diagrams/.cd, every~diagram,baseline={([yshift=-axis_height]\tikzcdmatrixname)}, #1]%
  \pgfsetlayers{background,quantback,main}%
    \tl_set:Nn \l_tmpa_tl {#2}%
    \tl_replace_all:Nnn \l_tmpa_tl { & } { \pgfmatrixnextcell }%
    \begingroup%doing it like this, we don't need to patch tikzcd, so it will continue to work independently.
      \def\tikzpicture[##1]{}%
      \let\endtikzpicture\relax%
      %bring in a bunch of stuff I used to introduce to tikzcd as a patch.
          \def\tikz@lib@matrix@empty@cell{%
      \iftikz@lib@matrix@empty\node[name=\tikzmatrixname-\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn,
      minimum~width=\ifcsundef{cell@width@\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}{0}{\csname cell@width@\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn\endcsname},
      minimum~height=\ifcsundef{cell@height@\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}{0}{\csname cell@height@\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn\endcsname}
      ]{};\wire{a}\fi
      \csgundef{cell@width@\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}
      \csgundef{cell@height@\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}}%
    %\pgfmathsetmacro{\mname}{random(100000)}
     \tikzcdset{%
  thick,
  nodes~in~empty~cells,
  every~cell/.style={
        anchor=center,minimum~size=0pt,inner~sep=0pt,outer~sep=0pt,thick,
        minimum~height=\ifcsundef{cell@height@\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}{0}{\csname cell@height@\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn\endcsname},
        minimum~width=\ifcsundef{cell@width@\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}{0}{\csname cell@width@\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn\endcsname},
        %append after command={\wire{a}}
        execute~at~end~cell={\wire{a}%looks promising. does not work on empty cells.
        %be careful to unset "global" variables that really only apply to current diagram
        \csgundef{cell@width@\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}
      \csgundef{cell@height@\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}
      \csgundef{wire@type@override@\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}}
    },
  arrowStyle/.style={dash,thick,line~cap=round},
  %1-row diagram/.style={},
  1-row~diagram/.style={/tikz/baseline={([yshift=-\MathAxis]\tikzcdmatrixname-1-1.center)}},%doesn't seem to be doing anything. Possibly activates too late?
  grade/.style={description,circle,draw,fill=white,inner~sep=0pt, outer~sep=0pt,font=\tiny}
}%
      \tikzcd[#1]%
    %\ifcsstring{toslice@qtkz}{1}{\ifcsstring{vert@qtkz}{0}{\pgfutil@g@addto@macro\tikzcd@atendslices\sliceallr}{\pgfutil@g@addto@macro\tikzcd@atendslices\sliceallvr}}{}%
      %\pgfutil@g@addto@macro\tikzcd@savedpaths{\begin{scope}[/tikz/commutative~diagrams/.cd,#1]}%
\l_tmpa_tl
      %\endtikzcd
      \pgfmatrixendrow\egroup%
  \pgfextra{\global\let\tikzcdmatrixname\tikzlastnode};%
  \tikzcdset{\the\pgfmatrixcurrentrow-row~diagram/.try}%
  \begingroup%
    \pgfkeys{% `quotes' library support
      /handlers/first~char~syntax/the~character~"/.initial=\tikzcd@forward@quotes,%
      /tikz/edge~quotes~mean={%
        edge~node={node [execute~at~begin~node=\iftikzcd@mathmode$\fi,%$
                         execute~at~end~node=\iftikzcd@mathmode$\fi,%$
                         /tikz/commutative~diagrams/.cd,every~label,##2]{##1}}}}%
    \let\tikzcd@errmessage\errmessage% improve error messages
    \def\errmessage##1{\tikzcd@errmessage{##1^^J...^^Jl.\tikzcd@lineno\space%
        I~think~the~culprit~is~a~tikzcd~arrow~in~cell~\tikzcd@currentrow-\tikzcd@currentcolumn}}%
    \tikzcd@before@paths@hook%
    \begin{pgfonlayer}{quantback}%
    \begingroup%
    \tikzcdset{wire~types/.code={}}%prevent setting of wire types, which wipes all the work we've done!
    %\begin{scope} already included in tikzcd@savedpaths so that it has right options
    \begin{scope}[/tikz/commutative~diagrams/.cd,#1]
    \ifcsstring{toslice@qtkz}{1}{\ifcsstring{vert@qtkz}{0}{\pgfutil@g@addto@macro\tikzcd@atendslices\sliceallr}{\pgfutil@g@addto@macro\tikzcd@atendslices\sliceallvr}}{}%
      \tikzcd@savedpaths
    \end{scope}
    \endgroup
    \end{pgfonlayer}
    \tikzcd@atendsavedpaths\tikzcd@atendlabels\tikzcd@atendslices%I just added stuff here instead
    \quantikz@endAltText
    \resetwiretypes%reset wire types
    \foreach \x in {1,...,\the\pgfmatrixcurrentrow} {
\foreach \y in {1,...,\the\pgfmatrixcurrentcolumn} {
\csgundef{wire@type@override@\x-\y}
\csgundef{cell@width@\x-\y}
}}
    \def\tikz@lib@matrix@empty@cell{\iftikz@lib@matrix@empty\node[name=\tikzmatrixname-\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn]{};\fi}%
  \endgroup%
  \endtikzpicture%
  \ifnum0=`{}\fi
    \endgroup
  \end{tikzpicture}
}{}
\ExplSyntaxOff




%patch tikzcd to allow for multiple layers of commands that get deferred until later
% \patchcmd\tikzcd@{\tikzpicture}{%
%   \def\toslice{0}\def\vert@qtkz{0}%
%  \begin{tikzpicture}}{}{}
%\patchcmd\tikzcd@{\tikzpicture[/tikz/commutative diagrams/.cd,every diagram,#1]}{%
%}{}{}
\patchcmd\tikzcd@
    {\global\let\tikzcd@savedpaths\pgfutil@empty}
    {\global\let\tikzcd@savedpaths\pgfutil@empty%
    \global\let\tikzcd@atendsavedpaths\pgfutil@empty%
    \global\let\tikzcd@atendlabels\pgfutil@empty%
    \global\let\tikzcd@atendslices\pgfutil@empty%
    \pgfutil@g@addto@macro\tikzcd@savedpaths\DivideRowsCols%
    }{}{}

%end patching

%%%%%%%%%%%%%%%%%%%%%%%
%
% define the keys
%
%%%%%%%%%%%%%%%%%%%%%%%
\pgfkeys{/quantikz/gates/.cd,%
  style/.store in=\quantikz@style,
  style={},
  Strike Width/.store in=\quantikz@sw,
  Strike Width=0.08cm,
  Strike Height/.store in=\quantikz@sh,
  Strike Height=0.12cm,
  label style/.store in=\quantikz@lstyle,
  label style={},
  wire style/.store in=\quantikz@wstyle,
  wire style={},
  vertical wire/.store in=\quantikz@wtype,
  vertical wire=q,
  partial swap/.store in=\quantikz@partial,
  partial swap={},
  partial position/.store in=\quantikz@pos,
  partial position=0.5,
  angle/.store in=\quantikz@angle,
  angle=-45,
  wires/.store in=\quantikz@wires,
  wires=1,
  row/.store in=\quantikz@row,
  row=1,
  col/.store in=\quantikz@col,
  col=1,
  priority label/.store in=\quantikz@priority,
  priority label={center},
  braces/.store in=\quantikz@braces,
  braces={},
  steps/.store in=\quantikz@steps,
  steps=1,
  ps/.store in=\quantikz@ps,
  ps={},
}
\pgfkeys{/tikz/commutative diagrams/.cd,%
 slice style/.store in=\quantikz@slicestyle,
 slice style={},
  slice label style/.store in=\quantikz@slicelstyle,
  slice label style={},
  slice titles/.store in=\quantikz@slicetitle,
  slice titles=\col,
}
%https://tex.stackexchange.com/a/524113/148934:
\tikzset{%
  set style/.style={#1},
  expand style/.style={%completely expands the <value> of its argument (using \edef) before processing the result as a <key>
    set style/.expanded={#1}% needs braces around the argument
  },
  expand style once/.style={%expands the <value> of its argument once before processing the result as a <key>
    set style/.expand once={#1}% needs braces around the argument
  },
  expand style twice/.style={%expands the <value> of its argument twice before processing the result as a <key>
    set style/.expand twice={#1}% needs braces around the argument
  }
}
%thanks to this, can store formats in macros such as \mystylelist, then apply
% \node[expand style once=\mystylelist] {B};
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% the basic wire command
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\ExplSyntaxOn
% take a direction, such as d and repeat it the required number of times
\NewExpandableDocumentCommand{\myrepeat}{O{}mm}
 {
  \int_compare:nT { #2 > 0 }
   {
    #3 \prg_replicate:nn { #2 - 1 } { #1#3 }
   }
 }
\ExplSyntaxOff

%this is the main entry point for people
%converts a wire command with distance into one using repeated letters (main directions only)
\NewDocumentCommand{\wire}{O{l}O{1}O{}m}{%direction (l/r/u/d), distance, decoration, quantum/classical/bundle/none
\ifstrequal{#2}{0}{%
\PackageWarning{quantikz}{You seem to have a wire of zero length. I believe the problem is in cell \the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}.
}{%
  \edef\length{\myrepeat{#2}{#1}}
\ifthenelse{\the\pgfmatrixcurrentcolumn>1}{%
\expandafter\fullwire\expandafter{\length}{#1}{#4}{#3}%
}{}
}}
%does the actual business of creating the different wire types with the correct anchors
%uses custom anchors on shapes for classical wires. We'll come to this in a minute.
\newcommand{\fullwire}[4]{%direction with repetition. direction. type. decoration
\edef\wiretype{#3}
\ifstrequal{#3}{a}{%automatic determination
  \ifcsundef{wire@type@\the\pgfmatrixcurrentrow}{%type not defined globally. assume quantum.
  \edef\wiretype{q}
  }{%
  \edef\wiretype{\csname wire@type@\the\pgfmatrixcurrentrow\endcsname}
  \ifdefstring{\wiretype}{u}{%
    \edef\wiretype{q}
  }{}
  }
  \ifcsdef{wire@type@override@\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}{%
    \edef\wiretype{\csname wire@type@override@\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn\endcsname}
  }{}
}{}
\ifdefstring{\wiretype}{q}{%quantum wire
    \arrow[#1,arrowStyle,#4] {}
  }{%
  \ifdefstring{\wiretype}{c}{%classical wire
    \arrow[arrowStyle,start anchor=#2startone,end anchor=#2endone] {#1}\arrow[arrowStyle,start anchor=#2starttwo,end anchor=#2endtwo,#4] {#1}
  }{%
  \ifdefstring{\wiretype}{b}{%wire bundle
    \arrow[arrowStyle,start anchor=#2startone,end anchor=#2endone,#4] {#1}\arrow[arrowStyle,start anchor=#2starttwo,end anchor=#2endtwo,#4] {#1}\arrow[#1,arrowStyle,#4] {}
  }{%
  \ifdefstring{\wiretype}{n}{%no wire
  }{\ifdefstring{\wiretype}{u}{%unset
  }{\PackageWarning{quantikz}{unknown wire type in cell \the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}}}}}}
}

\newcommand{\setwiretype}[2][\the\pgfmatrixcurrentrow]{%
%this command will record what the current wire type is supposed to be
\ifnumgreater{\the\pgfmatrixcurrentcolumn}{0}{%
\ifstrequal{#2}{c}{%
\quantikz@output{At time step \the\pgfmatrixcurrentcolumn, the type of wire for qubit \the\pgfmatrixcurrentrow\space changes to a classical wire.}
}{}
\ifstrequal{#2}{q}{%
\quantikz@output{At time step \the\pgfmatrixcurrentcolumn, the type of wire for qubit \the\pgfmatrixcurrentrow\space changes to a quantum wire.}
}{}
\ifstrequal{#2}{b}{%
\quantikz@output{At time step \the\pgfmatrixcurrentcolumn, the type of wire for qubit \the\pgfmatrixcurrentrow\space changes to a wire bundle.}
}{}
\ifstrequal{#2}{n}{%
\quantikz@output{At time step \the\pgfmatrixcurrentcolumn, the wire for qubit \the\pgfmatrixcurrentrow\space is removed.}
}{}
}{}
\ifstrequal{#2}{u}{
  \csgundef{wire@type@#1}
}{
\expandafter\gdef\csname wire@type@#1\endcsname{#2}%will need to reset all these variables at the beginning/end of a circuit.
}
}

\gdef\quantikz@alttext{0}
\newcommand{\quantikzAltText}[1]{%
%this command will set up an output system that we can hook into every time a quantikz circuit runs.
 \gdef\quantikz@alttext{1}
 \newwrite\quantikzoutput
 \immediate\openout\quantikzoutput=#1
 \immediate\write\quantikzoutput{Quantikz Alt Text}
}

\newcounter{alttextno}
\DeclareRobustCommand{\figAltText}[1]{%
%the alt text for the current environment (figure, table etc),\cref{current}, on page
%{\refstepcounter{alttextno}\label{alttext\thealttextno}}
\quantikz@output{}
\ifdefstring{\@currenvir}{figure}{%
{\refstepcounter{alttextno}\label{alttext\thealttextno}}
\quantikz@output{Alt text for Figure \thefigure\space on page \getpagerefnumber{alttext\thealttextno}.}
}{%
\ifdefstring{\@currenvir}{minipage}{%
\ifx\insidemargin\@undefined
   \quantikz@output{Alt text for Figure \thefigure\space on page \getpagerefnumber{alttext\thealttextno}.}%
\else
{\refstepcounter{alttextno}\label{alttext\thealttextno}}
   \quantikz@output{Alt text for the image in the margin of page \getpagerefnumber{alttext\thealttextno}.}%
\fi
}{%
{\refstepcounter{alttextno}\label{alttext\thealttextno}}
\quantikz@output{Alt text for the inline image on page \getpagerefnumber{alttext\thealttextno}.}
}
}
\quantikz@output{#1}
}

\newcommand{\quantikz@startAltText}{%
%per-circuit entry point
\ifthenelse{\quantikz@alttext=1}{%
\quantikz@output{}
\quantikz@output{Alt Text for quantum circuit on page \thepage. Unless stated otherwise, all wires carry quantum data (qubits).}
}{}
}

\newcommand{\quantikz@endAltText}{%
%per-circuit exit point
\ifthenelse{\quantikz@alttext=1}{%
\quantikz@output{This circuit has \the\pgfmatrixcurrentrow\space wires and \the\pgfmatrixcurrentcolumn\space time steps.}
}{}
}

\newcommand{\quantikz@output}[1]{%
\ifthenelse{\quantikz@alttext=1}{%
\immediate\write\quantikzoutput{#1}
}{}
}

\newcommand{\quantikzEndAltText}{%
\closeout\quantikzoutput  % to close the file
}

\NewDocumentCommand{\wireoverride}{O{\the\pgfmatrixcurrentrow}O{\the\pgfmatrixcurrentcolumn}m}{%
%change the wire type of this specific cell without unsetting the global wire type of this cell.
\expandafter\gdef\csname wire@type@override@#1-#2\endcsname{#3}
}

\newcommand{\wiretype}[1]{
  \ifstrequal{#1}{b}{a wire bundle}{}
  \ifstrequal{#1}{c}{a classical wire}{}
  \ifstrequal{#1}{n}{empty}{}
}

\newcounter{dummy}
\newcommand{\importwiretypes}[1]{%
%receive a list of wire types. Process them into individual variables
\setcounter{dummy}{1}% 
  \foreach \thiswire [count=\rownum] in {#1} {%
  \ifdefstring{\thiswire}{c}{%
    \quantikz@output{Wire \rownum\space is a classical wire.}
  }{}
  \ifdefstring{\thiswire}{b}{%
    \quantikz@output{Wire \rownum\space is a wire bundle.}
  }{}
  \ifdefstring{\thiswire}{n}{%
    \quantikz@output{Wire \rownum\space is blank.}
  }{}
    \expandafter\expandafter\expandafter\setwiretype\expandafter\expandafter\expandafter[\expandafter\rownum\expandafter]\expandafter{\thiswire}
    \stepcounter{dummy}
     }
     \pgfmathparse{\arabic{dummy}/2}
     %\pgfmathresult
     \expandafter\setmiddle\expandafter{\pgfmathresult}
  }%

\newcommand{\resetwiretypes}{%try to reset all definitions of per-row wire types
  \foreach \rownum in {1,...,\the\pgfmatrixcurrentrow} {%
\expandafter\setwiretype\expandafter[\rownum]{u} 
  }
}

\tikzset{%
  strike arrow/.style n args={3}{
    decoration={markings, mark=at position 0.5 with {
        \draw [internal,-] 
            ++ (#1, #2 )
            -- ( -#1, -#2) node [anchor=south west, inner sep=0pt] {$\scriptstyle #3$};} %can I use pgfkeys and do some maths here?
    },
    postaction={decorate},
}}
%this used to be a more complex command, but is now only used for adding the strikethrough + number
\newcommand{\qwbundle}[2][]{%
		%\ifthenelse{\the\pgfmatrixcurrentcolumn=2}{%do the strikethrough
  \pgfkeys{/quantikz/gates/.cd,style=,Strike Width=0.08cm,Strike Height=0.12cm,#1} 
  \edef\arg{strike arrow={\quantikz@sw}{\quantikz@sh}{#2},\quantikz@style}
			\expandafter\arrow\expandafter[\arg,phantom]{l}%
	}

%%%%%%%%%%%%%%%%%%%%%%%%%
%
% deprecated wire commands provided for backwards compatibility
%
%%%%%%%%%%%%%%%%%%%%%%%%%


%now add some of the basic wire commands for backwards compatibility. These should be largely superfluous once I'm done.
\newcommand{\vcw}[1]{%vertical classical wire. goes down by the amount specified in arg
\ifnumcomp{#1}{>}{0}{%
  \wire[d][#1]{c}
}{\ifnumcomp{#1}{<}{0}{%
  \wire[u][-#1]{c}
}{\PackageWarning{quantikz}{You seem to have a vertical classical wire with no height in cell \the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn!}}}
}
%vertical quantum wire, relative positioning
\newcommand{\vqw}[1]{
\ifnumcomp{#1}{>}{0}{%
  \wire[d][#1]{q}
}{\ifnumcomp{#1}{<}{0}{%
  \wire[u][-#1]{q}
}{\PackageWarning{quantikz}{You seem to have a vertical quantum wire with no height in cell \the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn!}}}
}

%basic horzontal quantum wire, length 1. Goes backwards 1 cell. Won't do anything in the first cell.
\newcommand{\qw}{\wire{q}}
%basic horzontal classical wire, length 1. Goes backwards 1 cell. Won't do anything in the first cell.
\newcommand{\cw}{\wire{c}}
%use for fudging classical wires that have horizontal and vertical sections
%shouldn't really be necessary any more?
\NewExpandableDocumentCommand{\cwbend}{m}{
  \phase{}\vcw{#1}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% shape definitions
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%we will mainly be using rectangle and circle as base shapes. Also signal, rounded rectangle for some measurement objects. cross out for swap.
%First we need to add custom anchors to them for attaching the wires.

%helper functions
\newcommand*\pgfdeclareanchoralias[3]{%
    \expandafter\def\csname pgf@anchor@#1@#3\expandafter\endcsname
            \expandafter{\csname pgf@anchor@#1@#2\endcsname}}
\def\pgfaddtoshape#1#2{%
  \begingroup
  \def\pgf@sm@shape@name{#1}%
  \let\anchor\pgf@sh@anchor
  #2%
  \endgroup
}

%add anchors to the rectangle
\pgfaddtoshape{rectangle}{%
    \anchor{dendtwo}{%
    \pgf@process{\southwest}%
    \pgf@xa=.5\pgf@x%
    \pgf@process{\northeast}%
    \pgf@x=.5\pgf@x%
    \advance\pgf@x by \pgf@xa%
    \advance\pgf@x by \pgfkeysvalueof{/tikz/commutative diagrams/classical gap horizontal}%
  }%
  \anchor{dstarttwo}{%
    \pgf@process{\northeast}%
    \pgf@xa=.5\pgf@x%
    \pgf@process{\southwest}%
    \pgf@x=.5\pgf@x%
    \advance\pgf@x by \pgf@xa%
    \advance\pgf@x by \pgfkeysvalueof{/tikz/commutative diagrams/classical gap horizontal}%
  }%
  \anchor{dendone}{%
    \pgf@process{\southwest}%
    \pgf@xa=.5\pgf@x%
    \pgf@process{\northeast}%
    \pgf@x=.5\pgf@x%
    \advance\pgf@x by \pgf@xa%
    \advance\pgf@x by -\pgfkeysvalueof{/tikz/commutative diagrams/classical gap horizontal}%
  }%
  \anchor{dstartone}{%
    \pgf@process{\northeast}%
    \pgf@xa=.5\pgf@x%
    \pgf@process{\southwest}%
    \pgf@x=.5\pgf@x%
    \advance\pgf@x by \pgf@xa%
    \advance\pgf@x by -\pgfkeysvalueof{/tikz/commutative diagrams/classical gap horizontal}%
  }%
    \anchor{lstarttwo}{%
    \pgf@process{\northeast}%
    \pgf@ya=.5\pgf@y%
    \pgf@process{\southwest}%
    \pgf@y=.5\pgf@y%
    \advance\pgf@y by \pgf@ya%
    \advance\pgf@y by \pgfkeysvalueof{/tikz/commutative diagrams/classical gap vertical}%
  }%
  \anchor{lendtwo}{%
    \pgf@process{\southwest}%
    \pgf@ya=.5\pgf@y%
    \pgf@process{\northeast}%
    \pgf@y=.5\pgf@y%
    \advance\pgf@y by \pgf@ya%
    \advance\pgf@y by \pgfkeysvalueof{/tikz/commutative diagrams/classical gap vertical}%
  }%
  \anchor{lstartone}{%
    \pgf@process{\northeast}%
    \pgf@ya=.5\pgf@y%
    \pgf@process{\southwest}%
    \pgf@y=.5\pgf@y%
    \advance\pgf@y by \pgf@ya%
    \advance\pgf@y by -\pgfkeysvalueof{/tikz/commutative diagrams/classical gap vertical}%
  }%
  \anchor{lendone}{%
    \pgf@process{\southwest}%
    \pgf@ya=.5\pgf@y%
    \pgf@process{\northeast}%
    \pgf@y=.5\pgf@y%
    \advance\pgf@y by \pgf@ya%
    \advance\pgf@y by -\pgfkeysvalueof{/tikz/commutative diagrams/classical gap vertical}%
  }%
  }
\pgfdeclareanchoralias{rectangle}{dendtwo}{ustarttwo}
\pgfdeclareanchoralias{rectangle}{dendone}{ustartone}
\pgfdeclareanchoralias{rectangle}{dstarttwo}{uendtwo}
\pgfdeclareanchoralias{rectangle}{dstartone}{uendone}
\pgfdeclareanchoralias{rectangle}{lendtwo}{rstarttwo}
\pgfdeclareanchoralias{rectangle}{lendone}{rstartone}
\pgfdeclareanchoralias{rectangle}{lstarttwo}{rendtwo}
\pgfdeclareanchoralias{rectangle}{lstartone}{rendone}

%add anchors to the circle
\pgfaddtoshape{circle}{%
  \anchor{dstartone}{
    \centerpoint
    \pgf@xa=\radius
    \advance\pgf@x by-\pgfkeysvalueof{/tikz/commutative diagrams/classical gap horizontal}
    \ifdimgreater{\pgfkeysvalueof{/tikz/commutative diagrams/classical gap horizontal}}{\radius}{%
\PackageError{quantikz}{You have tried to create a control object with classical control wire, but "classical gap horizontal" is set too large.}{Change the environment parameter for the quantikz environment using the "classical gap horizontal=" key to a value smaller than 0.06cm.}
    }{}
    \pgfmathparse{-sqrt(\radius*\radius-\pgfkeysvalueof{/tikz/commutative diagrams/classical gap horizontal}*\pgfkeysvalueof{/tikz/commutative diagrams/classical gap horizontal})}
    \advance\pgf@y by\pgfmathresult pt
  }%
  \anchor{dstarttwo}{
    \centerpoint
    \pgf@xa=\radius
    \ifdimgreater{\pgfkeysvalueof{/tikz/commutative diagrams/classical gap horizontal}}{\radius}{%
\PackageError{quantikz}{You have tried to create a control object with classical control wire, but "classical gap horizontal" is set too large.}{Change the environment parameter for the quantikz environment using the "classical gap hoirzontal=" key to a value smaller than 0.06cm.}
    }{}
    \advance\pgf@x by\pgfkeysvalueof{/tikz/commutative diagrams/classical gap horizontal}
    \pgfmathparse{-sqrt(\radius*\radius-\pgfkeysvalueof{/tikz/commutative diagrams/classical gap horizontal}*\pgfkeysvalueof{/tikz/commutative diagrams/classical gap horizontal})}
    \advance\pgf@y by\pgfmathresult pt
  }%
  \anchor{dendone}{
    \centerpoint
    \pgf@xa=\radius
    \ifdimgreater{\pgfkeysvalueof{/tikz/commutative diagrams/classical gap horizontal}}{\radius}{%
\PackageError{quantikz}{You have tried to create a control object with classical control wire, but "classical gap horizontal" is set too large.}{Change the environment parameter for the quantikz environment using the "classical gap horizontal=" key to a value smaller than 0.06cm.}
    }{}
    \advance\pgf@x by-\pgfkeysvalueof{/tikz/commutative diagrams/classical gap horizontal}
    \pgfmathparse{sqrt(\radius*\radius-\pgfkeysvalueof{/tikz/commutative diagrams/classical gap horizontal}*\pgfkeysvalueof{/tikz/commutative diagrams/classical gap horizontal})}
    \advance\pgf@y by\pgfmathresult pt
  }%
  \anchor{dendtwo}{
    \centerpoint
    \pgf@xa=\radius
    \ifdimgreater{\pgfkeysvalueof{/tikz/commutative diagrams/classical gap horizontal}}{\radius}{%
\PackageError{quantikz}{You have tried to create a control object with classical control wire, but "classical gap horizontal" is set too large.}{Change the environment parameter for the quantikz environment using the "classical gap horizontal=" key to a value smaller than 0.06cm.}
    }{}
    \advance\pgf@x by\pgfkeysvalueof{/tikz/commutative diagrams/classical gap horizontal}
    \pgfmathparse{sqrt(\radius*\radius-\pgfkeysvalueof{/tikz/commutative diagrams/classical gap horizontal}*\pgfkeysvalueof{/tikz/commutative diagrams/classical gap horizontal})}
    \advance\pgf@y by\pgfmathresult pt
  }%
  \anchor{lstartone}{
    \centerpoint
    \pgf@xa=\radius
    \ifdimgreater{\pgfkeysvalueof{/tikz/commutative diagrams/classical gap vertical}}{\radius}{%
\PackageError{quantikz}{You have tried to create a control object with classical control wire, but "classical gap vertical" is set too large.}{Change the environment parameter for the quantikz environment using the "classical gap vertical=" key to a value smaller than 0.06cm.}
    }{}
    \advance\pgf@y by-\pgfkeysvalueof{/tikz/commutative diagrams/classical gap vertical}
    \pgfmathparse{-sqrt(\radius*\radius-\pgfkeysvalueof{/tikz/commutative diagrams/classical gap vertical}*\pgfkeysvalueof{/tikz/commutative diagrams/classical gap vertical})}
    \advance\pgf@x by\pgfmathresult pt
  }%
  \anchor{lstarttwo}{
    \centerpoint
    \pgf@xa=\radius
    \ifdimgreater{\pgfkeysvalueof{/tikz/commutative diagrams/classical gap vertical}}{\radius}{%
\PackageError{quantikz}{You have tried to create a control object with classical control wire, but "classical gap vertical" is set too large.}{Change the environment parameter for the quantikz environment using the "classical gap vertical=" key to a value smaller than 0.06cm.}
    }{}
    \advance\pgf@y by\pgfkeysvalueof{/tikz/commutative diagrams/classical gap vertical}
    \pgfmathparse{-sqrt(\radius*\radius-\pgfkeysvalueof{/tikz/commutative diagrams/classical gap vertical}*\pgfkeysvalueof{/tikz/commutative diagrams/classical gap vertical})}
    \advance\pgf@x by\pgfmathresult pt
  }%
  \anchor{lendone}{
    \centerpoint
    \pgf@xa=\radius
    \ifdimgreater{\pgfkeysvalueof{/tikz/commutative diagrams/classical gap vertical}}{\radius}{%
\PackageError{quantikz}{You have tried to create a control object with classical control wire, but "classical gap vertical" is set too large.}{Change the environment parameter for the quantikz environment using the "classical gap vertical=" key to a value smaller than 0.06cm.}
    }{}
    \advance\pgf@y by-\pgfkeysvalueof{/tikz/commutative diagrams/classical gap vertical}
    \pgfmathparse{sqrt(\radius*\radius-\pgfkeysvalueof{/tikz/commutative diagrams/classical gap vertical}*\pgfkeysvalueof{/tikz/commutative diagrams/classical gap vertical})}
    \advance\pgf@x by\pgfmathresult pt
  }%
  \anchor{lendtwo}{
    \centerpoint
    \pgf@xa=\radius
    \ifdimgreater{\pgfkeysvalueof{/tikz/commutative diagrams/classical gap vertical}}{\radius}{%
\PackageError{quantikz}{You have tried to create a control object with classical control wire, but "classical gap vertical" is set too large.}{Change the environment parameter for the quantikz environment using the "classical gap vertical=" key to a value smaller than 0.06cm.}
    }{}
    \advance\pgf@y by\pgfkeysvalueof{/tikz/commutative diagrams/classical gap vertical}
    \pgfmathparse{sqrt(\radius*\radius-\pgfkeysvalueof{/tikz/commutative diagrams/classical gap vertical}*\pgfkeysvalueof{/tikz/commutative diagrams/classical gap vertical})}
    \advance\pgf@x by\pgfmathresult pt
  }%
}
\pgfdeclareanchoralias{circle}{dendtwo}{ustarttwo}
\pgfdeclareanchoralias{circle}{dendone}{ustartone}
\pgfdeclareanchoralias{circle}{dstarttwo}{uendtwo}
\pgfdeclareanchoralias{circle}{dstartone}{uendone}
\pgfdeclareanchoralias{circle}{lendtwo}{rstarttwo}
\pgfdeclareanchoralias{circle}{lendone}{rstartone}
\pgfdeclareanchoralias{circle}{lstarttwo}{rendtwo}
\pgfdeclareanchoralias{circle}{lstartone}{rendone}

\pgfaddtoshape{rounded rectangle}{%
%I'm going to cheat and assume it's always wide enough to have a flat bottom/top.
	\anchor{dstartone}{%
 		\roundedrectanglepoints%
 		\pgfpointadd{\centerpoint}{\pgfpoint{-\pgfkeysvalueof{/tikz/commutative diagrams/classical gap horizontal}}{-\halfheight-\outerysep}}%
	}
	\anchor{dstarttwo}{%
 		\roundedrectanglepoints%
 		\pgfpointadd{\centerpoint}{\pgfpoint{\pgfkeysvalueof{/tikz/commutative diagrams/classical gap horizontal}}{-\halfheight-\outerysep}}%
	}
	\anchor{dendone}{%
 		\roundedrectanglepoints%
 		\pgfpointadd{\centerpoint}{\pgfpoint{-\pgfkeysvalueof{/tikz/commutative diagrams/classical gap horizontal}}{\halfheight+\outerysep}}%
	}
	\anchor{dendtwo}{%
 		\roundedrectanglepoints%
 		\pgfpointadd{\centerpoint}{\pgfpoint{\pgfkeysvalueof{/tikz/commutative diagrams/classical gap horizontal}}{\halfheight+\outerysep}}%
	}
	\anchor{lstarttwo}{%
	\roundedrectanglepoints%
    \ifx\westarc\pgf@lib@sh@misc@rr@text@concave%
    %not sure! Just leave it. I don't think even the simple quantum wire works as I want it out the box!
    \pgfpointadd{\centerpoint}{\pgfpoint{-\halfwidth-\outerxsep}{\pgfkeysvalueof{/tikz/commutative diagrams/classical gap vertical}}}%
        % \pgfpathlineto{\pgfpoint{-\halfwidth-\arcwidth}{+-\halfheight}}%
        % \pgfpatharc{+-\halfarcangle}{+\halfarcangle}{+\radius}%
    \else%
        \ifx\westarc\pgf@lib@sh@misc@rr@text@convex%
        		\pgfextract@process\arccenter{%
               	\pgfpointadd{\centerpoint}{\pgfpoint{-\halfwidth-\chordwidth+\radius}{+0pt}}%
            }%
            \pgfmathparse{sqrt((\radius+\outerxsep)^2-\pgfkeysvalueof{/tikz/commutative diagrams/classical gap vertical}^2)}
            \pgfpointadd{\arccenter}{\pgfpoint{-\pgfmathresult pt}{\pgfkeysvalueof{/tikz/commutative diagrams/classical gap vertical}}}
        \else%
            \pgfpointadd{\centerpoint}{\pgfpoint{-\halfwidth-\outerxsep}{\pgfkeysvalueof{/tikz/commutative diagrams/classical gap vertical}}}%
        \fi%
    \fi%
	}
	\anchor{lstartone}{%
	\roundedrectanglepoints%
   \ifx\westarc\pgf@lib@sh@misc@rr@text@concave%
    %not sure!
    \pgfpointadd{\centerpoint}{\pgfpoint{-\halfwidth-\outerxsep}{-\pgfkeysvalueof{/tikz/commutative diagrams/classical gap vertical}}}%
    %     % \pgfpathlineto{\pgfpoint{-\halfwidth-\arcwidth}{+-\halfheight}}%
    %     % \pgfpatharc{+-\halfarcangle}{+\halfarcangle}{+\radius}%
    \else%
        \ifx\westarc\pgf@lib@sh@misc@rr@text@convex%
        		\pgfextract@process\arccenter{%
               	\pgfpointadd{\centerpoint}{\pgfpoint{-\halfwidth-\chordwidth+\radius}{+0pt}}%
            }%
            \pgfmathparse{sqrt((\radius+\outerxsep)^2-\pgfkeysvalueof{/tikz/commutative diagrams/classical gap vertical}^2)}
            \pgfpointadd{\arccenter}{\pgfpoint{-\pgfmathresult pt}{-\pgfkeysvalueof{/tikz/commutative diagrams/classical gap vertical}}}
        \else%
            \pgfpointadd{\centerpoint}{\pgfpoint{-\halfwidth-\outerxsep}{-\pgfkeysvalueof{/tikz/commutative diagrams/classical gap vertical}}}%
        \fi%
    \fi%
	}	
	\anchor{lendtwo}{%
	\roundedrectanglepoints%
    \ifx\eastarc\pgf@lib@sh@misc@rr@text@concave%
    %not sure!
        % \pgfpathlineto{\pgfpoint{-\halfwidth-\arcwidth}{+-\halfheight}}%
        % \pgfpatharc{+-\halfarcangle}{+\halfarcangle}{+\radius}%
    \else%
        \ifx\eastarc\pgf@lib@sh@misc@rr@text@convex%
        		\pgfextract@process\arccenter{%
               	\pgfpointadd{\centerpoint}{\pgfpoint{\halfwidth+\chordwidth-\radius}{+0pt}}%
            }%
            \pgfmathparse{sqrt((\radius+\outerxsep)^2-\pgfkeysvalueof{/tikz/commutative diagrams/classical gap vertical}^2)}
            \pgfpointadd{\arccenter}{\pgfpoint{\pgfmathresult pt}{\pgfkeysvalueof{/tikz/commutative diagrams/classical gap vertical}}}
            %\pgfpathlineto{\pgfpoint{-\halfwidth-\chordwidth+\arcwidth}{+-\halfheight}}%
            %\pgfpatharc{180+\halfarcangle}{180-\halfarcangle}{+\radius}%
        \else%
            \pgfpointadd{\centerpoint}{\pgfpoint{\halfwidth}{\pgfkeysvalueof{/tikz/commutative diagrams/classical gap vertical}}}%
        \fi%
    \fi%
	}
	\anchor{lendone}{%
	\roundedrectanglepoints%
    \ifx\eastarc\pgf@lib@sh@misc@rr@text@concave%
    %not sure!
        % \pgfpathlineto{\pgfpoint{-\halfwidth-\arcwidth}{+-\halfheight}}%
        % \pgfpatharc{+-\halfarcangle}{+\halfarcangle}{+\radius}%
    \else%
        \ifx\eastarc\pgf@lib@sh@misc@rr@text@convex%
        		\pgfextract@process\arccenter{%
               	\pgfpointadd{\centerpoint}{\pgfpoint{\halfwidth+\chordwidth-\radius}{+0pt}}%
            }%
            \pgfmathparse{sqrt((\radius+\outerxsep)^2-\pgfkeysvalueof{/tikz/commutative diagrams/classical gap vertical}^2)}
            \pgfpointadd{\arccenter}{\pgfpoint{\pgfmathresult pt}{-\pgfkeysvalueof{/tikz/commutative diagrams/classical gap vertical}}}
            %\pgfpathlineto{\pgfpoint{-\halfwidth-\chordwidth+\arcwidth}{+-\halfheight}}%
            %\pgfpatharc{180+\halfarcangle}{180-\halfarcangle}{+\radius}%
        \else%
            \pgfpointadd{\centerpoint}{\pgfpoint{\halfwidth}{-\pgfkeysvalueof{/tikz/commutative diagrams/classical gap vertical}}}%
        \fi%
    \fi%
	}
	}
\pgfdeclareanchoralias{rounded rectangle}{dendtwo}{ustarttwo}
\pgfdeclareanchoralias{rounded rectangle}{dendone}{ustartone}
\pgfdeclareanchoralias{rounded rectangle}{dstarttwo}{uendtwo}
\pgfdeclareanchoralias{rounded rectangle}{dstartone}{uendone}
\pgfdeclareanchoralias{rounded rectangle}{lendtwo}{rstarttwo}
\pgfdeclareanchoralias{rounded rectangle}{lendone}{rstartone}
\pgfdeclareanchoralias{rounded rectangle}{lstarttwo}{rendtwo}
\pgfdeclareanchoralias{rounded rectangle}{lstartone}{rendone}


\pgfaddtoshape{signal}{%
	\anchor{lstarttwo}{%
		\installsignalparameters
		\let\firstpoint\anchornorthwest
		\let\secondpoint\anchorwest
    \pgfpointintersectionoflines%
      {\firstpoint}%
      {\secondpoint}%
      {\pgfpointadd{\secondpoint}{\pgfpoint{0cm}{\pgfkeysvalueof{/tikz/commutative diagrams/classical gap vertical}}}}%
      {\pgfpointadd{\secondpoint}{\pgfpoint{0.5cm}{\pgfkeysvalueof{/tikz/commutative diagrams/classical gap vertical}}}}%
	}
	\anchor{lstartone}{%
		\installsignalparameters
		\let\firstpoint\anchorsouthwest
		\let\secondpoint\anchorwest
		\pgfpointintersectionoflines%
      {\firstpoint}%
      {\secondpoint}%
      {\pgfpointadd{\secondpoint}{\pgfpoint{0cm}{-\pgfkeysvalueof{/tikz/commutative diagrams/classical gap vertical}}}}%
      {\pgfpointadd{\secondpoint}{\pgfpoint{0.5cm}{-\pgfkeysvalueof{/tikz/commutative diagrams/classical gap vertical}}}}%
	}
	\anchor{lendtwo}{%
		\installsignalparameters
		\let\firstpoint\anchornortheast
		\let\secondpoint\anchoreast
    \pgfpointintersectionoflines%
      {\firstpoint}%
      {\secondpoint}%
      {\pgfpointadd{\secondpoint}{\pgfpoint{0cm}{-\pgfkeysvalueof{/tikz/commutative diagrams/classical gap vertical}}}}%
      {\pgfpointadd{\secondpoint}{\pgfpoint{0.5cm}{-\pgfkeysvalueof{/tikz/commutative diagrams/classical gap vertical}}}}%
	}
	\anchor{lendone}{%
		\installsignalparameters
		\let\firstpoint\anchorsoutheast
		\let\secondpoint\anchoreast
    \pgfpointintersectionoflines%
      {\firstpoint}%
      {\secondpoint}%
      {\pgfpointadd{\secondpoint}{\pgfpoint{0cm}{\pgfkeysvalueof{/tikz/commutative diagrams/classical gap vertical}}}}%
      {\pgfpointadd{\secondpoint}{\pgfpoint{0.5cm}{\pgfkeysvalueof{/tikz/commutative diagrams/classical gap vertical}}}}%
	}
  \anchor{dstarttwo}{%
  	\installsignalparameters
    \pgf@process{\southanchor}%
    \advance\pgf@x by \pgfkeysvalueof{/tikz/commutative diagrams/classical gap horizontal}%
  }%
  \anchor{dstartone}{%
  	\installsignalparameters
    \pgf@process{\southanchor}%
    \advance\pgf@x by -\pgfkeysvalueof{/tikz/commutative diagrams/classical gap horizontal}%
  }%
  \anchor{dendtwo}{%
  	\installsignalparameters
    \pgf@process{\northanchor}%
    \advance\pgf@x by \pgfkeysvalueof{/tikz/commutative diagrams/classical gap horizontal}%
  }%
  \anchor{dendone}{%
  	\installsignalparameters
    \pgf@process{\northanchor}%
    \advance\pgf@x by -\pgfkeysvalueof{/tikz/commutative diagrams/classical gap horizontal}%
  }%}
 }
\pgfdeclareanchoralias{signal}{dendtwo}{ustarttwo}
\pgfdeclareanchoralias{signal}{dendone}{ustartone}
\pgfdeclareanchoralias{signal}{dstarttwo}{uendtwo}
\pgfdeclareanchoralias{signal}{dstartone}{uendone}
\pgfdeclareanchoralias{signal}{lendtwo}{rstarttwo}
\pgfdeclareanchoralias{signal}{lendone}{rstartone}
\pgfdeclareanchoralias{signal}{lstarttwo}{rendtwo}
\pgfdeclareanchoralias{signal}{lstartone}{rendone}

% if these base shapes won't do, you'll have to create your own definition, either of a whole shape or take an existing one and add extra anchors, as above.
% you need to make sure that the anchor border works correctly for lines approaching from the 4 compass points, as these are where the quantum wires attach.
% classical wires instead attach to points that are displaced by a horizontal/vertical amount \pgfkeysvalueof{/tikz/commutative diagrams/classical gap} relative to these positions. These are called:
% dstartone,dstarttwo,dendone,dendtwo
% ustartone,ustarttwo,uendone,uendtwo
% lstartone,lstarttwo,lendone,lendtwo
% rstartone,rstarttwo,rendone,rendtwo
%The idea, for example, is if you have an "l" type classical wire, there will be two wires, one going from lstartone (the left-hand edge on your shape, \pgfkeysvalueof{/tikz/commutative diagrams/classical gap} vertically above the west anchor) and going to lendone (l end one) on the cell one to the left. Typically, you expect lendone and rstartone to be the same points. There is also a line from lstarttwo to lendtwo.

% often the shape you want can just be a modification of an existing shape. Critically, the border should be the same. Then we don't need to define a whole new shape, we can just do it with styles. Much easier!

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% gate definitions
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%single qubit operations
%\tikzset{linecont/.style={line}}
\newcommand{\phantomgate}[1]{|[line,thickness, inner sep=4pt,minimum width=1.5pt,minimum height=1.5pt]| \phantom{#1}}
\newcommand{\hphantomgate}[1]{|[line,minimum size=1.5em, inner xsep=4pt,thickness]| \hphantom{#1}}
\newcommand{\linethrough}{|[line,thickness, inner ysep=3pt]| }
\newcommand{\push}[1]{#1}
%\newcommand{\alias}[1]{|[alias=#1]|}

\tikzset{
circle phase/.style={fill,shape=circle,minimum size=0.12cm,draw},
rrectangle phase/.style={fill,shape=rectangle,rounded corners=1.5pt,minimum width=3pt,minimum height=2.5*\pgfkeysvalueof{/tikz/commutative diagrams/classical gap vertical}+3pt,draw},
phase/.code={%
  \pgfkeys{/quantikz/gates/.cd,style=,label style=,#1}%
  \ifcsundef{wire@type@\the\pgfmatrixcurrentrow}{%type not defined globally. assume quantum.
    \edef\wiretype{q}
  }{%
    \edef\wiretype{\csname wire@type@\the\pgfmatrixcurrentrow\endcsname}
  }
  \ifcsstring{wiretype}{b}{\ifdimless{\pgfkeysvalueof{/tikz/commutative diagrams/classical gap vertical}}{0.04cm}{\tikzset{circle phase}}{\tikzset{rrectangle phase}}}{%
    \ifcsstring{wiretype}{c}{\ifdimless{\pgfkeysvalueof{/tikz/commutative diagrams/classical gap vertical}}{0.04cm}{\tikzset{circle phase}}{\tikzset{rrectangle phase}}}{\tikzset{circle phase}}
  }
  \expandafter\tikzset\expandafter{\quantikz@style}
  \pgfkeys{/quantikz/gates/.cd,style=,label style=,#1}%run again so that "open" can take priority
  },
phase label/.code={\tikzset{label distance=2mm,anchor=mid,label position=45}
  \pgfkeys{/quantikz/gates/.cd,style=,label style=,#1}%
  \edef\quantikz@style{\quantikz@style,\quantikz@lstyle}
  \expandafter\tikzset\expandafter{\quantikz@style}
},
}

\DeclareExpandableDocumentCommand{\phase}{O{}m}{|[phase={#1},label={[phase label={#1}]#2}]| {}\quantikz@output{Qubit \the\pgfmatrixcurrentrow\space has a phase gate applied at time step \the\pgfmatrixcurrentcolumn\space of phase #1.}}
\DeclareExpandableDocumentCommand{\control}{O{}m}{|[phase={#1}]| {}\quantikz@output{Qubit \the\pgfmatrixcurrentrow\space is the control of a gate at time step \the\pgfmatrixcurrentcolumn.}}
\DeclareExpandableDocumentCommand{\ocontrol}{O{}m}{\control[open,#1]{}}
%\DeclareExpandableDocumentCommand{\ocontrol}{O{}m}{|[phase={#1,open}]| {}}
\DeclareExpandableDocumentCommand{\targ}{O{}m}{|[circlewc={#1}]| {}\quantikz@output{Qubit \the\pgfmatrixcurrentrow\space is the target of a controlled not operation at time step \the\pgfmatrixcurrentcolumn.}}
\DeclareExpandableDocumentCommand{\targX}{O{}m}{|[crossx2={#1}]| {}}


\tikzset{
	cross/.style={path picture={ 
		\draw[internal](path picture bounding box.north) -- (path picture bounding box.south) (path picture bounding box.west) -- (path picture bounding box.east);
	}},
  circlewc/.code={
  \tikzset{draw,circle,cross,minimum width=4pt,inner sep=3pt}
    \pgfkeys{/quantikz/gates/.cd,style=,#1}%
    \expandafter\tikzset\expandafter{\quantikz@style}
  },
  crossx/.style={path picture={ 
		\draw[internal,inner sep=0pt]
		(path picture bounding box.south east) -- (path picture bounding box.north west) (path picture bounding box.south west) -- (path picture bounding box.north east); %(path picture bounding box.west) -- (path picture bounding box.east);
	}},
  crossdraw/.pic = {
    \begin{pgfinterruptboundingbox}
      \node[cross out,draw,minimum size=0.7em,#1] {};
    \end{pgfinterruptboundingbox}
  },
  crossx2/.code={
    \pgfkeys{/quantikz/gates/.cd,style=,#1}%
    \edef\styling{crossx3=\quantikz@style}
    \expandafter\tikzset\expandafter{\styling}
  },
  crossx3/.style={
    append after command={
      (\tikzlastnode.center) pic{crossdraw={#1}}
    }
  }
}

%%%
%
%measuring
%
%%%

%standard meter device
%first, define the styles
\tikzset{
  meter/.style={draw,
    %fill=\pgfkeysvalueof{/tikz/commutative diagrams/background color},
    filling,
    minimum width=2em,
    minimum height=1.5em,
    rectangle, 
    font=\vphantom{A}, 
    thickness,
    path picture={
        \draw ([shift={(.1,-.06)}]path picture bounding box.west) to[bend left=50] ([shift={(-.1,-.06)}]path picture bounding box.east);
        \draw[-{Latex[scale=0.6]}] ([shift={(0,-.1)}]path picture bounding box.center) -- ([shift={(-.1,.2)}]path picture bounding box.east);
    },
    },
    my label/.style={yshift=0.1cm,above,align=center},
}
%\DeclareExpandableDocumentCommand{\meter}{O{}{m}}{|[meter,label={[my label]#2},#1]| {}}
% \DeclareExpandableDocumentCommand{\meter}{O{}O{1.5pt}O{1.5pt}m}{%
% \gate[priority label={above},priority style={meter},#1][#2][#3]{#4}
% }
\DeclareExpandableDocumentCommand{\meter}{O{}O{2em}O{1.5em}m}{%
\gate[#1,priority label=above,disable auto height,ps=meter][#2][#3]{#4}
}
%code not working here :( Either I can get my predefined label style to apply, or the user's custom style. Not both.

\newcommand{\meterout}[1]{
\quantikz@output{The following output is a measurement outcome for the previous measurement.}
\rstick{$#1$}\setwiretype{n}\ar[l,leftarrow]{}
}

%gate variant with classical result wire
\tikzset{
    metercw/.style={draw=none,
    yshift=0.375em,
        fill=none,
        minimum width=2em,
        minimum height=2.25em,
        font=\vphantom{A}, 
        thickness,
        path picture={
        %if you draw the rectangle to be the full width of the box, you cut off half the line, so have to bring it in a little.
        \node[draw,thickness,filling,#1,inner sep=0pt, minimum height=0pt,minimum width=0pt,fit={([shift={(.5\pgflinewidth,.5\pgflinewidth)}]path picture bounding box.south west) ([shift={(-.5\pgflinewidth,-0.75em)}]path picture bounding box.north east)}] (rect) {};
        %  \draw [#1]([xshift={0.5\pgflinewidth}]path picture bounding box.south west) rectangle ([yshift=-0.75em,xshift={-0.5\pgflinewidth}]path picture bounding box.north east);
          %draw the two classical wires
          \draw ([xshift=\pgfkeysvalueof{/tikz/commutative diagrams/classical gap horizontal},yshift=-0.75em]path picture bounding box.north) -- ([xshift=\pgfkeysvalueof{/tikz/commutative diagrams/classical gap horizontal}]path picture bounding box.north);
          \draw ([xshift=-\pgfkeysvalueof{/tikz/commutative diagrams/classical gap horizontal},yshift=-0.75em]path picture bounding box.north) -- ([xshift=-\pgfkeysvalueof{/tikz/commutative diagrams/classical gap horizontal}]path picture bounding box.north);
          %draw the image in the middle of the box
            \draw ([shift={(.1,-.06)}]rect.west) to[bend left=50] ([shift={(-.1,-.06)}]rect.east);
        \draw[-{Latex[scale=0.6]}] ([shift={(0,-.1)}]rect.center) -- ([shift={(-.1,.2)}]rect.east);
        }
    }
}
%\DeclareExpandableDocumentCommand{\metercw}{O{}{m}}{|[metercw={#1},label={[my labelcw]#2}]| {}}
\DeclareExpandableDocumentCommand{\metercw}{O{}O{2em}O{2.25em}m}{%
\gate[#1,priority label=above,ps=metercw,disable auto height][#2][#3]{#4}
}

\tikzset{measuretab/.style={draw,signal,signal to=west,filling,minimum width=2em, minimum height=1em,inner sep=4pt}}
\DeclareExpandableDocumentCommand{\measuretab}{O{}{m}}{|[measuretab,#1]| {#2}}
%considered making this a multiqubit gate, but any non-straight edge works badly with incoming wires and transparency.
%it might be that your use case is tolerable.
% \DeclareExpandableDocumentCommand{\measuretab}{O{}O{2em}O{1.5pt}m}{%
% \gate[#1,ps=measuretab][#2][#3]{#4}
% }

\tikzset{
  meterD/.style={
        draw,
        shape=rounded rectangle,
        rounded rectangle west arc=none,
        inner sep=4pt,
        filling
    },
  inputD/.style={
        draw,
        shape=rounded rectangle,
        rounded rectangle east arc=none,
        inner sep=4pt,
        filling
    }
}
%should these have a multi-qubit option?
\DeclareExpandableDocumentCommand{\meterD}{O{}{m}}{|[meterD,#1]| {#2}}
\DeclareExpandableDocumentCommand{\inputD}{O{}{m}}{|[inputD,#1]| {#2}\wireoverride{n}}
% \DeclareExpandableDocumentCommand{\meterD}{O{}O{1.5pt}O{1.5pt}m}{%
% \gate[#1,ps=meterD][#2][#3]{#4}
% }
\tikzset{measure/.style={draw=black,rounded rectangle,filling, minimum width=2em, minimum height=1em, inner sep=4pt}}

% \DeclareExpandableDocumentCommand{\measure}{O{}O{2em}O{1.5pt}m}{%
% \gate[#1,ps=measure][#2][#3]{#4}
% }

\DeclareExpandableDocumentCommand{\measure}{O{}{m}}{|[measure,#1]| {#2}}


\tikzset{trash/.style={path picture={
    \edef\yshift{\pgfkeysvalueof{/tikz/commutative diagrams/classical gap vertical}}
    \ifcsstring{wire@type@\the\pgfmatrixcurrentrow}{c}{%
      \draw[internal,inner sep=0pt,-stealth] ([yshift={\yshift}]path picture bounding box.west) -- ([yshift={\yshift}]path picture bounding box.center) -- (path picture bounding box.south);
      \draw[internal,inner sep=0pt] ([yshift={-\yshift}]path picture bounding box.west) -- ([yshift={-\yshift}]path picture bounding box.center);
    }{%
      \draw[internal,inner sep=0pt,-stealth] (path picture bounding box.west) -- (path picture bounding box.center) -- (path picture bounding box.south);
      \ifcsstring{wire@type@\the\pgfmatrixcurrentrow}{b}{%
        \draw[internal,inner sep=0pt] ([yshift={\yshift}]path picture bounding box.west) -- ([yshift={\yshift}]path picture bounding box.center) -- (path picture bounding box.center);
        \draw[internal,inner sep=0pt] ([yshift={-\yshift}]path picture bounding box.west) -- ([yshift={-\yshift}]path picture bounding box.center);
      }{}
    }
    %\edef\yshift{\pgfkeysvalueof{/tikz/commutative diagrams/classical gap}}
    },
    minimum height=2.5em,
    minimum width=2em}}

\DeclareExpandableDocumentCommand{\trash}{O{}{m}}{|[trash,label={below:#2},#1]| {}}

\tikzset{ground/.style={path picture={
    \draw[internal,inner sep=0pt]([xshift={0.5\pgflinewidth}]path picture bounding box.south west) -- ([xshift={0.5\pgflinewidth}]path picture bounding box.north west);
    \draw[internal,inner sep=0pt]([xshift={0.5\pgflinewidth+2*\pgfkeysvalueof{/tikz/commutative diagrams/classical gap horizontal}},yshift={\pgfkeysvalueof{/tikz/commutative diagrams/classical gap vertical}}]path picture bounding box.south west) -- ([xshift={0.5\pgflinewidth+2*\pgfkeysvalueof{/tikz/commutative diagrams/classical gap horizontal}},yshift={-\pgfkeysvalueof{/tikz/commutative diagrams/classical gap vertical}}]path picture bounding box.north west);
    \draw[internal,inner sep=0pt]([xshift={0.5\pgflinewidth+4*\pgfkeysvalueof{/tikz/commutative diagrams/classical gap horizontal}},yshift={2*\pgfkeysvalueof{/tikz/commutative diagrams/classical gap vertical}}]path picture bounding box.south west) -- ([xshift={0.5\pgflinewidth+4*\pgfkeysvalueof{/tikz/commutative diagrams/classical gap horizontal}},yshift={-2*\pgfkeysvalueof{/tikz/commutative diagrams/classical gap vertical}}]path picture bounding box.north west);
  },
  minimum height=8*\pgfkeysvalueof{/tikz/commutative diagrams/classical gap vertical},
  minimum width=5*\pgfkeysvalueof{/tikz/commutative diagrams/classical gap horizontal}
  }}
\DeclareExpandableDocumentCommand{\ground}{O{}{m}}{|[ground,label={below:#2},#1]| {}}
%\DeclareExpandableDocumentCommand{\bin}{O{}{m}}{|[bin,label={below:#2},#1]| {}}

%\newlength{\boxsize}
%\setlength{\boxsize}{\maxof{\pgfkeysvalueof{/tikz/commutative diagrams/classical gap horizontal}}{\pgfkeysvalueof{/tikz/commutative diagrams/classical gap vertical}}}
%this may take some fixing if classical gap horizontal != classical gap vertical
\tikzset{cbend/.style={
    path picture={
    \draw[internal,inner sep=0pt,thick] ($(path picture bounding box.#1)+cos(#1)*(0,-\pgfkeysvalueof{/tikz/commutative diagrams/classical gap vertical})+sin(#1)*(\pgfkeysvalueof{/tikz/commutative diagrams/classical gap horizontal},0)$) arc (270+#1:180+#1:3*\pgfkeysvalueof{/tikz/commutative diagrams/classical gap horizontal} and 3*\pgfkeysvalueof{/tikz/commutative diagrams/classical gap vertical});
    \draw[internal,inner sep=0pt,thick] ($(path picture bounding box.#1)+cos(#1)*(0,\pgfkeysvalueof{/tikz/commutative diagrams/classical gap vertical})+sin(#1)*(-\pgfkeysvalueof{/tikz/commutative diagrams/classical gap horizontal},0)$) arc (270+#1:180+#1:\pgfkeysvalueof{/tikz/commutative diagrams/classical gap horizontal} and \pgfkeysvalueof{/tikz/commutative diagrams/classical gap vertical});
  },
  minimum height=4*\pgfkeysvalueof{/tikz/commutative diagrams/classical gap vertical},
  minimum width=4*\pgfkeysvalueof{/tikz/commutative diagrams/classical gap horizontal},
  }}
\NewExpandableDocumentCommand{\cbend}{m}{
|[cbend=#1]| {}
}

% \def\bin{\begin{tikzpicture}[thickness,scale=0.2]
%\draw (0,0) -- (1,0) -- (1,-0.2) -- (2,-0.8) -- (1.4,-3) -- (-0.4,-3) -- (-1,-0.8) -- (0,-0.2) -- cycle;
% \draw (2,-0.8) arc (360:180:1.5 and 0.2);
% \draw (-0.2,-1.1) -- (0.3,-2.8);
% \draw (1.2,-1.1) -- (0.7,-2.8);
% \end{tikzpicture}}


%%%
%
%controlled gates
%
%%%

\NewExpandableDocumentCommand{\ctrl}{O{}m}{\control[#1]{}%
  \pgfkeys{/quantikz/gates/.cd,style=,label style=,wire style=,vertical wire=q,#1}%
  \edef\style{\quantikz@style,\quantikz@wstyle}
\ifthenelse{\equal{#2}{}}{}{%empty parameter should be equivalent to 0
\ifnumequal{#2}{0}{%do nothing
}{%otherwise draw a wire
\ifnumgreater{#2}{0}{%down wires
   \expandafter\expandafter\expandafter\expandedwire\expandafter\expandafter\expandafter{\expandafter\style\expandafter}\expandafter{\quantikz@wtype}{d}{#2}
   \IfSubStr{#1}{open}{%
\quantikz@output{A gate is controlled off qubit \the\pgfmatrixcurrentrow\space at time step \the\pgfmatrixcurrentcolumn, targeting its action on a qubit #2 below it when the present qubit is in the 0 state.}
   }{%
   \quantikz@output{A gate is controlled off qubit \the\pgfmatrixcurrentrow\space at time step \the\pgfmatrixcurrentcolumn, targeting a qubit #2 below it.}
   }
% %  \wire[d][#2][\style]{\wtype}
}{%up wires
  \expandafter\expandafter\expandafter\expandedwire\expandafter\expandafter\expandafter{\expandafter\style\expandafter}\expandafter{\quantikz@wtype}{u}{-#2}
     \IfSubStr{#1}{open}{%
\quantikz@output{A gate is controlled off qubit \the\pgfmatrixcurrentrow\space at time step \the\pgfmatrixcurrentcolumn, targeting its action on a qubit -#2 above it when the present qubit is in the 0 state.}
   }{%
   \quantikz@output{A gate is controlled off qubit \the\pgfmatrixcurrentrow\space at time step \the\pgfmatrixcurrentcolumn, targeting a qubit -#2 above it.}
   }
%  \wire[u][-#3][#2]{#1}
}
}}
}
\NewExpandableDocumentCommand{\octrl}{O{}m}{\ctrl[#1,open]{#2}}

\NewDocumentCommand\expandedwire{mmmm}{\wire[#3][#4][#1]{#2}} % this basically lets me put the things that need expanding first

\DeclareExpandableDocumentCommand{\swap}{O{}m}{%styling,label of partial swap, displacement of partial swap, distance
|[crossx2={#1}]| {}
\IfInteger{#2}{%allgood
}{%
\PackageWarning{quantikz}{You have asked for a swap gate in cell \the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn\ that should span a non-integer number of wires! Could you have forgotten the pair of curly braces at the end?}
}
\pgfkeys{/quantikz/gates/.cd,partial swap=,style=,partial position=0.5,label style=,vertical wire=q,#1}%
\ifnumequal{#2}{0}{%don't bother trying to draw a wire
}{%
\ifdefempty{\quantikz@partial}{%
  \edef\tempstyle{\quantikz@style}
%   \expandafter\vqw\expandafter[\opts]{#2}
  }{%
%   %\pgfkeysgetvalue{/quantikz/gates/label style}{\labstyle}
  \ifdefstring{\wtype}{c}{%
\edef\tempstyle{"{\quantikz@partial}"{grade,pos=\quantikz@pos,\quantikz@lstyle,xshift=-\pgfkeysvalueof{/tikz/commutative diagrams/classical gap horizontal}},\quantikz@style}
  }{%
  \edef\tempstyle{"{\quantikz@partial}"{grade,pos=\quantikz@pos,\quantikz@lstyle},\quantikz@style}
  }
%   \expandafter\expandedwire\expandafter{\tempstyle}{q}{d}{#2}
%   %\wire[d][#3][\tempstyle]{q}
  }
 \expandafter\expandafter\expandafter\expandedwire\expandafter\expandafter\expandafter{\expandafter\tempstyle\expandafter}\expandafter{\quantikz@wtype}{d}{#2}
}
}



%misc
\DeclareDocumentCommand{\makeebit}{O{}m}{
  \pgfkeys{/quantikz/gates/.cd,style=,label style=,angle=-45,#1}%
  \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\make@ebit\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\quantikz@style\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\quantikz@lstyle\expandafter}\expandafter{\quantikz@angle}{#2}
  %\arrow[arrows,line cap=round,\style,to path={(\tikztostart) -- ($(\tikztostart)!{0.5/cos(\angle)}!\angle:(\tikztotarget)$) node [anchor=east,style={\lstyle}]{#2} -- (\tikztotarget) }]{d}
}
\DeclareDocumentCommand{\make@ebit}{mmmm}{%
  \arrow[arrowStyle,line cap=round,#1,to path={(\tikztostart) --  ($(\tikztostart)!{0.5/cos(#3)}!#3:(\tikztotarget)$) node [anchor=east,style={#2}]{#4} --(\tikztotarget) }]{d}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% helpers
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\newlength{\myl}
\newlength{\myh}
\newlength{\myd}

%\makeatletter
\newcounter{aaa}
\tikzset{
  apply/.style args={#1 except on segments #2}{postaction={
      /utils/exec={
        \@for\mattempa:=#2\do{\csdef{aaa@\mattempa}{}}
        \setcounter{aaa}{0}
      },
      decorate,decoration={show path construction,
        moveto code={},
        lineto code={
          \stepcounter{aaa}
          \ifcsdef{aaa@\theaaa}{}{
            \path[#1] (\tikzinputsegmentfirst) -- (\tikzinputsegmentlast);
          }
        },
        curveto code={
          \stepcounter{aaa}
          \ifcsdef{aaa@\theaaa}{}{
            \path [#1] (\tikzinputsegmentfirst) .. controls
            (\tikzinputsegmentsupporta) and (\tikzinputsegmentsupportb)
            ..(\tikzinputsegmentlast);
          }
        },
        closepath code={
          \stepcounter{aaa}
          \ifcsdef{aaa@\theaaa}{}{
            \path [#1] (\tikzinputsegmentfirst) -- (\tikzinputsegmentlast);
          }
        },
      },
    },
  },
}


%
%commands for putting in text vertically (e.g. for slices)
\protected\def\verticaltext#1{\leavevmode\bgroup\vbox\bgroup\xvvv#1\relax}
%
\def\xvvv{\afterassignment\xxvvv\let\tmp= }
%
\def\xxvvv{%
% \ifx\tmp\@sptoken\egroup\ \vbox\bgroup\let\next\xvvv
% \else
\ifx\tmp\relax\egroup\egroup\let\next\relax
 \else
\hbox to 1.1em{\hfill\tmp\hfill}% centred
\let\next\xvvv\fi%\fi
\next}
%end of commands for putting text vertically
%
\long\def\ifnodedefined#1#2#3{%
    \@ifundefined{pgf@sh@ns@#1}{#3}{#2}%
}

%find the vertical position of the middle of an equals sign
%https://tex.stackexchange.com/questions/355680/how-can-i-vertically-align-an-equals-sign-in-a-tikz-node/355686
\pgfmathsetmacro\MathAxis{height("$\vcenter{}$")}



\newcounter{wirenumberpermute}

\newcommand{\permute}[1]{%
\hphantom{Wide}%
\def\firstlist{#1}
\edef\n{\the\pgfmatrixcurrentrow} %the row
  \edef\m{\the\pgfmatrixcurrentcolumn} %the column
\edef\keys{row=\n,col=\m}
 	\edef\mn{\the\numexpr\m-1\relax}
 	\edef\mp{\the\numexpr\m+1\relax}
 	\settowidth{\myl}{$Wide$}
 	\setcounter{wirenumberpermute}{0}
 	\foreach \x [count=\c] in \firstlist {%
 		\edef\start{\the\numexpr\c+\n-1\relax}%
 		\edef\endy{\the\numexpr\x+\n-1\relax}%
 		%apply auto width to the cell, and make sure we unset the setting so that it doesn't apply to later circuits.
    \csxdef{cell@width@\start-\m}{\the\myl} %save the cell width for every row in a global variable
 		\stepcounter{wirenumberpermute}
 	 	}
 	 	\expandafter\pgfutil@g@addto@macro\expandafter\tikzcd@atendsavedpaths\expandafter{%
 	 	\expandafter\wirepair@end\expandafter{\keys}{#1}%
 		}
 	\edef\lim{\the\numexpr\arabic{wirenumberpermute}+\n-1\relax}
 	 	\foreach \i in {\n,...,\lim} {%
 	     \edef\newcom{\noexpand\vqwexplicit{\i-\m}{\i-\mn}}
 	 		 \newcom%
 	 	}
}

\newcommand{\wirepair@end}[2]{%#row,col of left-most site. #row of right-most site.
  \pgfkeys{/quantikz/gates/.cd,#1}
	\xdef\LoopGG{}
	\edef\i{\quantikz@row}
	\def\firstlist{#2}
	%\show\i
	%\show\j
	%create a list of cell names to be included in this grouped gate
	\foreach \n in \firstlist {%
	\ifnodedefined{\tikzcdmatrixname-\the\numexpr\n+\i-1\relax-\quantikz@col}{%
		\xdef\LoopGG{\LoopGG(\tikzcdmatrixname-\the\numexpr\n+\i-1\relax-\quantikz@col)}
		}{}
	}
	\ifnodedefined{\tikzcdmatrixname-\i-\quantikz@col}{%
		\xdef\LoopGG{\LoopGG(\tikzcdmatrixname-\i-\quantikz@col)}
		}{}
	\node (group\tikzcdmatrixname-\quantikz@row-\quantikz@col) [fit=\LoopGG,transparent,inner sep=0pt] {\phantom{Wide}};
		\foreach \n [count=\c] in \firstlist{%
			\draw [line width=3pt,\pgfkeysvalueof{/tikz/commutative diagrams/background color},shorten >=0.9pt,shorten <=0.9pt] (group\tikzcdmatrixname-\quantikz@row-\quantikz@col.west|-\tikzcdmatrixname-\the\numexpr\i+\c-1\relax-\quantikz@col.center) to[out=0,in=180] (group\tikzcdmatrixname-\quantikz@row-\quantikz@col.east|-\tikzcdmatrixname-\the\numexpr\i+\n-1\relax-\quantikz@col.center);
			\draw [thickness] (group\tikzcdmatrixname-\quantikz@row-\quantikz@col.west|-\tikzcdmatrixname-\the\numexpr\i+\c-1\relax-\quantikz@col.center) to[out=0,in=180] (group\tikzcdmatrixname-\quantikz@row-\quantikz@col.east|-\tikzcdmatrixname-\the\numexpr\i+\n-1\relax-\quantikz@col.center);
		}
}


%%%
%
%the main gate command
%
%%%

\DeclareExpandableDocumentCommand{\gate}{O{}O{1.5pt}O{1.5pt}m}{%optional parameter contains styling info. compulsory is gate text.
	|[inner sep=4pt,minimum width=#2,minimum height=#3]|%
 	\edef\n{\the\pgfmatrixcurrentrow} %the row
 	\edef\m{\the\pgfmatrixcurrentcolumn} %the column
 	%reset macros that are going to be set by the options
 	\edef\options{row=\n,col=\m,#1}
 	\def\toswap{0}%
 	\def\DisableMinSize{0}%
 	%\pgfkeys{/quantikz,wires=1,style=,label style=,braces=}%
 	%import options passed as parameters
  	\pgfkeys{/quantikz/gates/.cd,wires=1,style=,label style=,braces=,#1}%
  \ifnumless{\quantikz@wires}{0}{%
    \PackageError{quantikz}{You cannot have a gate command with a negative number of wires. The culprit appears to be cell \the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}
    }{%
      \ifnumequal{\quantikz@wires}{0}{%
        \PackageError{quantikz}{You cannot have a gate command with 0 wires. The culprit appears to be cell \the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}
      }{}
      }
  %\pgfkeys{/quantikz/gates/style/.estyle={\pgfkeysvalueof{/quantikz/gates/ps},\pgfkeysvalueof{/quantikz/gates/style},meter}}
  % {\pgfkeysvalueof{/quantikz/gates/ps},\quantikz@style
 	\ifthenelse{\toswap=1}{%if it's a swap gate...
  \ifnumequal{\quantikz@wires}{2}{%good!
  \quantikz@output{At time step \the\pgfmatrixcurrentcolumn, a swap gate is applied between qubit \the\pgfmatrixcurrentrow and the next.}
  }{%
  \PackageWarning{quantikz}{You have asked for a swap gate in cell \the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn. This required the number of wires that the gate acts on to be overridden. Check this is your intended behaviour}
 		\pgfkeys{/quantikz/gates/wires=2}
    }
 		\phantom{wide}
 		\settowidth{\myl}{$wide$}
 		\settoheight{\myh}{$wide$}
 		\settodepth{\myd}{$wide$}
 	}{%not a swap gate
  %figure out how large the per-cell box should be
 		\settowidth{\myl}{$#4$}
 		\ifthenelse{\DisableMinSize=1}{%disable automatic size detection. Use $U$ instead.
 			\phantom{U}
 			\settoheight{\myh}{$U$}
 			\settodepth{\myd}{$U$}
 		}{%automatically get width and height of label
 			\phantom{#4}
 			\settoheight{\myh}{$#4$}
 			\settodepth{\myd}{$#4$}
 		}
 	}
%	communicate per-cell sizes to the other cells
 	\edef\k{\the\numexpr\n+\quantikz@wires-1\relax}
% 	\edef\mn{\the\numexpr\m-1\relax}
  \ifnumgreater{\quantikz@wires}{1}{%
  \IfSubStr{#1}{ps=meter}{%
\quantikz@output{At time step \the\pgfmatrixcurrentcolumn, a measurement is applied to qubits \the\pgfmatrixcurrentrow to \k.}
  }{%
  \quantikz@output{At time step \the\pgfmatrixcurrentcolumn, a gate \unexpanded{#4} is applied to qubits \the\pgfmatrixcurrentrow\space to \k.}
  }
 	\foreach \i in {\the\numexpr\n+1\relax,...,\k} {
    \csxdef{cell@width@\i-\m}{max(\the\myl+8pt,#2)} %save the cell width for every row in a global variable
 	}
  \csxdef{cell@height@\k-\m}{max(\the\myh+\the\myd+8pt,#3)} %apply auto height to last row only.
%		
 	}{%
  \IfSubStr{#1}{ps=meter}{%
\quantikz@output{At time step \the\pgfmatrixcurrentcolumn, a measurement is applied to qubit \the\pgfmatrixcurrentrow.}
  }{%
  \quantikz@output{At time step \the\pgfmatrixcurrentcolumn, a gate \unexpanded{#4} is applied to qubit \the\pgfmatrixcurrentrow.}
  }
  }
 	%call deferred gate command. to be executed after the tikzcd matrix stuff is completed
	\expandafter\pgfutil@g@addto@macro\expandafter\tikzcd@atendsavedpaths\expandafter{%
		\expandafter\gate@end\expandafter{\options}{#4}
	}
}

%deferred gate command. draws a box around all included cells. this is not part of the matrix, but comes afterwards.
\newcommand{\gate@end}[2]{
	\pgfkeys{/quantikz/gates/.cd,wires=1,ps=,label style=,style=,priority label={center}}
	\def\toswap{0}
	\def\DisableMinSize{0}
 	\pgfkeys{/quantikz/gates/.cd,#1}%import options
  %\pgfkeys{/quantikz/gates/.cd,style=meter}
  %\pgfkeyssetevalue{/quantikz/gates/style}{\pgfkeysvalueof{/quantikz/gates/ps},\pgfkeysvalueof{/quantikz/gates/style}}
	\ifthenelse{\toswap=1}{%
\pgfkeys{/quantikz/gates/wires=2}
 }{}
	\xdef\LoopGG{}
	%create a list of cell names to be included in this grouped gate
	\foreach \n in  {\quantikz@row,...,\the\numexpr\quantikz@row+\quantikz@wires-1\relax} {
	\ifnodedefined{\tikzcdmatrixname-\n-\quantikz@col}{
		\xdef\LoopGG{\LoopGG(\tikzcdmatrixname-\n-\quantikz@col)}
		}{}
	}
	\ifthenelse{\toswap=1}{%
		\node (group\tikzcdmatrixname-\quantikz@row-\quantikz@col) [fit=\LoopGG,operator,inner sep=0pt,expand style once=\quantikz@ps,expand style once=\quantikz@style] {\hphantom{Wide}};
		\draw [thickness] (group\tikzcdmatrixname-\quantikz@row-\quantikz@col.west|-\tikzcdmatrixname-\quantikz@row-\quantikz@col.center) to[out=0,in=180] (group\tikzcdmatrixname-\quantikz@row-\quantikz@col.east|-\tikzcdmatrixname-\the\numexpr\quantikz@row+1\relax-\quantikz@col.center);
		\draw [line width=3pt,\pgfkeysvalueof{/tikz/commutative diagrams/background color},shorten >=0.9pt,shorten <=0.9pt] (group\tikzcdmatrixname-\quantikz@row-\quantikz@col.east|-\tikzcdmatrixname-\quantikz@row-\quantikz@col.center) to[out=180,in=0] (group\tikzcdmatrixname-\quantikz@row-\quantikz@col.west|-\tikzcdmatrixname-\the\numexpr\quantikz@row+1\relax-\quantikz@col.center);
		\draw [thickness] (group\tikzcdmatrixname-\quantikz@row-\quantikz@col.east|-\tikzcdmatrixname-\quantikz@row-\quantikz@col.center) to[out=180,in=0] (group\tikzcdmatrixname-\quantikz@row-\quantikz@col.west|-\tikzcdmatrixname-\the\numexpr\quantikz@row+1\relax-\quantikz@col.center);
	}{%
% 	%the actual gate drawing command
	  \node (group\tikzcdmatrixname-\quantikz@row-\quantikz@col) [fit=\LoopGG,operator,inner sep=0pt,label={[gg label,expand style once=\quantikz@lstyle]\quantikz@priority:$#2$},expand style once=\quantikz@ps,expand style once=\quantikz@style] {\hphantom{$#2$}};
	}
}

%ghost will get height correct if can't be automatically assigned.
\DeclareExpandableDocumentCommand{\ghost}{O{0pt}O{1.5pt}m}{%optional parameter contains styling info. compulsory is gate text.
	|[inner ysep=4pt,minimum width=#1,minimum height=#2]| \vphantom{#3}
}

%%%
%
%slicing
%
%%%

%single slice
\newcommand\slice[2][]{%
	%\edef\currcol{\the\pgfmatrixcurrentcolumn}
	%
 	%\edef\options{\quantikz@slicestyle,\quantikz@style}
 	%\edef\opts{\quantikz@slicelstyle,\quantikz@lstyle}
	\edef\n{\the\pgfmatrixcurrentcolumn}
	%\expandafter\show\n
	\expandafter\pgfutil@g@addto@macro\expandafter\tikzcd@atendslices\expandafter{%
		\expandafter\slice@end\expandafter{\n}{#1}{#2}%
	}}
%deferred slice command
\newcommand{\slice@end}[3]{
\quantikz@output{A vertical slice has been added at time step #1.}
	\edef\top{($1/2*(\tikzcdmatrixname-col#1.east |- \tikzcdmatrixname-row1.north)+1/2*(\tikzcdmatrixname-col\the\numexpr#1+1\relax.west |- \tikzcdmatrixname-row1.north)$)}
	\edef\bottom{($1/2*(\tikzcdmatrixname-col#1.east |- \tikzcdmatrixname-row\the\pgfmatrixcurrentrow.south)+1/2*(\tikzcdmatrixname-col\the\numexpr#1+1\relax.west |- \tikzcdmatrixname-row\the\pgfmatrixcurrentrow.south)+(0,-3pt)$)}
	\expandafter\expandafter\expandafter\make@slice\expandafter\expandafter\expandafter{\expandafter\top\expandafter}\expandafter{\bottom}{#3}{#2}
}
\newcommand{\make@slice}[4]{
  \pgfkeys{/quantikz/gates/.cd,wires=1,style=,label style=,braces=}
  \pgfkeys{/quantikz/gates/.cd,#4}%
	\draw[slice,expand style once=\quantikz@slicestyle,expand style once=\quantikz@style] #1 to node[pos=0,inner sep=4pt,anchor=south,color=black,expand style once=\quantikz@slicelstyle,expand style once=\quantikz@lstyle] {#3} #2;
}
%deferred command which will slice everything
\newcommand{\sliceallr}{%
\quantikz@output{A vertical slice has been added at every time step.}
	\foreach \n in  {2,...,\the\numexpr\pgfmatrixcurrentcolumn-1-\pgfkeysvalueof{/tikz/commutative diagrams/remove end slices}\relax} {
		\edef\col{\the\numexpr\n-1\relax}
		\expandafter\slice@end\expandafter{\n}{}{\quantikz@slicetitle}
	}
}
%deferred slice command with vertical text
\newcommand{\sliceallvr}{
	\foreach \n in  {2,...,\the\numexpr\pgfmatrixcurrentcolumn-1-\pgfkeysvalueof{/tikz/commutative diagrams/remove end slices}\relax} {
		\edef\col{\the\numexpr\n-1\relax}
		\edef\title{\verticaltext{\quantikz@slicetitle}}
		\expandafter\slice@end\expandafter{\n}{}{\title}
	}
}

%labelling of inputs
\newcommand{\lstick}[2][]{%
%\wlog{\tikzcdmatrixname}
	\pgfkeys{/quantikz/gates/.cd,wires=1,style=,label style=,braces=,#1}%
	\edef\newoptions{row=\the\pgfmatrixcurrentrow,col=\the\pgfmatrixcurrentcolumn,#1}
   \ifnumless{\quantikz@wires}{0}{%
    \PackageError{quantikz}{You cannot have an lstick command with a negative number of wires. The culprit appears to be cell \the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}
    }{%
      \ifnumequal{\quantikz@wires}{0}{%
        \PackageError{quantikz}{You cannot have an lstick command with 0 wires. The culprit appears to be cell \the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}
      }{}
      }
      \ifnumgreater{\quantikz@wires}{1}{%
\quantikz@output{The input state of \quantikz@wires\space qubits starting from qubit \the\pgfmatrixcurrentrow\space is \unexpanded{#2}.}
      }{%
\quantikz@output{The input state of qubit \the\pgfmatrixcurrentrow\space is \unexpanded{#2}.}
      }
	%\edef\n{\the\pgfmatrixcurrentrow}
	%\edef\m{\the\pgfmatrixcurrentcolumn}
	\expandafter\pgfutil@g@addto@macro\expandafter\tikzcd@atendsavedpaths\expandafter{%
		\expandafter\groupinput@end\expandafter{\newoptions}{#2}%
	}
}
\newcommand{\ifcsstringeitheror}[4]{%
\ifcsstring{#1}{#2}{#4}{\ifcsstring{#1}{#3}{#4}{}}
}
%deferred labelling of inputs
\newcommand{\groupinput@end}[2]{%basic data as keys, label options, brace options, text
  %\pgfkeys{/quantikz/gates/.cd,wires=1}%
  \def\rightbrace{1}%
  \pgfkeys{/quantikz/gates/.cd,wires=1,label style=,style=,braces=,#1}%
  \xdef\LoopGI{}
  \ifcsstringeitheror{wire@type@\quantikz@row}{c}{b}{%is the first wire classical? (should include bundle as well)
\xdef\LoopGI{\LoopGI($(\tikzcdmatrixname-\quantikz@row-\quantikz@col.center)+(0,\pgfkeysvalueof{/tikz/commutative diagrams/classical gap vertical})$)}
  }
   \ifcsstringeitheror{wire@type@\the\numexpr\quantikz@row+\quantikz@wires-1\relax}{c}{b}{%is the last wire classical? (should include bundle as well)
\xdef\LoopGI{\LoopGI($(\tikzcdmatrixname-\the\numexpr\quantikz@row+\quantikz@wires-1\relax-\quantikz@col.center)+(0,-\pgfkeysvalueof{/tikz/commutative diagrams/classical gap vertical})$)}
  }
  \foreach \n in  {\quantikz@row,...,\the\numexpr\quantikz@row+\quantikz@wires-1\relax} {
  \ifnodedefined{\tikzcdmatrixname-\n-\quantikz@col}{
    \xdef\LoopGI{\LoopGI(\tikzcdmatrixname-\n-\quantikz@col)} 
    }{}
    }
  \ifnumequal{\quantikz@wires}{1} {%
    \node (ingr-\quantikz@row) [fit=\LoopGI, inner sep=0pt,label={[align=center,expand style once=\quantikz@lstyle]left:#2}] {};
  }{%
  \node (ingr-\quantikz@row) [fit=\LoopGI, inner sep=0pt,label={[align=center,anchor=east,xshift=-0.2cm,expand style once=\quantikz@lstyle]left:#2}] {};
  \ifnumequal{\rightbrace}{1}{
  \draw[dm,expand style once=\quantikz@braces] ($(ingr-\quantikz@row.north west)+(-0.1cm,0.1cm)$) to ($(ingr-\quantikz@row.south west)+(-0.1cm,-0.1cm)$);
  }{}
 }
} %
%labelling of outputs
\newcommand\rstick[2][]{%
	\pgfkeys{/quantikz/gates/.cd,wires=1,style=,label style=,braces=,#1}%
	\edef\newoptions{row=\the\pgfmatrixcurrentrow,col=\the\pgfmatrixcurrentcolumn,#1}
   \ifnumless{\quantikz@wires}{0}{%
    \PackageError{quantikz}{You cannot have an rstick command with a negative number of wires. The culprit appears to be cell \the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}
    }{%
      \ifnumequal{\quantikz@wires}{0}{%
        \PackageError{quantikz}{You cannot have an rstick command with 0 wires. The culprit appears to be cell \the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}
      }{}
      }
	%\edef\n{\the\pgfmatrixcurrentrow}
	%\edef\m{\the\pgfmatrixcurrentcolumn}
  \ifnumequal{\quantikz@wires}{1}{%
  \quantikz@output{The final state of qubit \the\pgfmatrixcurrentrow, at time step \the\pgfmatrixcurrentcolumn, is \unexpanded{#2}.}
  }{%
\quantikz@output{The final state of the \quantikz@wires\space qubits starting with qubit \the\pgfmatrixcurrentrow, at time step \the\pgfmatrixcurrentcolumn, is \unexpanded{#2}.}
  }
	\expandafter\pgfutil@g@addto@macro\expandafter\tikzcd@atendsavedpaths\expandafter{%
		\expandafter\groupoutput@end\expandafter{\newoptions}{#2}%
	}
}
%deferred labelling of outputs
\newcommand{\groupoutput@end}[2]{%basic data as keys, label options, brace options, text
  \pgfkeys{/quantikz/gates/.cd,wires=1}
  \def\leftbrace{1}
  \pgfkeys{/quantikz/gates/.cd,#1}%
  \xdef\LoopGO{}
    \ifcsstringeitheror{wire@type@\quantikz@row}{c}{b}{%is the first wire classical? (should include bundle as well)
\xdef\LoopGO{\LoopGO($(\tikzcdmatrixname-\quantikz@row-\quantikz@col.center)+(0,\pgfkeysvalueof{/tikz/commutative diagrams/classical gap vertical})$)}
  }
   \ifcsstringeitheror{wire@type@\the\numexpr\quantikz@row+\quantikz@wires-1\relax}{c}{b}{%is the last wire classical? (should include bundle as well)
\xdef\LoopGO{\LoopGO($(\tikzcdmatrixname-\the\numexpr\quantikz@row+\quantikz@wires-1\relax-\quantikz@col.center)+(0,-\pgfkeysvalueof{/tikz/commutative diagrams/classical gap vertical})$)}
  }
  \foreach \n in  {\quantikz@row,...,\the\numexpr\quantikz@row+\quantikz@wires-1\relax} {
    \ifnodedefined{\tikzcdmatrixname-\n-\quantikz@col}{
      \xdef\LoopGO{\LoopGO(\tikzcdmatrixname-\n-\quantikz@col)} 
    }}
    \ifnumequal{\quantikz@wires}{1} {
    \node (outgr-\quantikz@row) [fit=\LoopGO, inner sep=0pt,label={[align=center,expand style once=\quantikz@lstyle]right:#2}] {};
  }{
  \node (outgr-\quantikz@row) [fit=\LoopGO, inner sep=0pt,label={[align=center,anchor=west,xshift=0.2cm,expand style once=\quantikz@lstyle]left:#2}] {};
  \ifthenelse{\leftbrace=1}{
  \draw[dd,expand style once=\quantikz@braces] ($(outgr-\quantikz@row.north east)+(0.1cm,0.1cm)$) to ($(outgr-\quantikz@row.south east)+(0.1cm,-0.1cm)$);
  }{}
  }
} %
\newcommand\midstick[2][]{%
	\hphantom{\text{g#2g}}\ %leave enough space for whatever text we've inserted
	\pgfkeys{/quantikz/gates/.cd,wires=1,style=,label style=,braces=,#1}%
	\edef\newoptions{row=\the\pgfmatrixcurrentrow,col=\the\pgfmatrixcurrentcolumn,#1}
   \ifnumless{\quantikz@wires}{0}{%
    \PackageError{quantikz}{You cannot have a midstick command with a negative number of wires. The culprit appears to be cell \the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}
    }{%
      \ifnumequal{\quantikz@wires}{0}{%
        \PackageError{quantikz}{You cannot have a midstick command with 0 wires. The culprit appears to be cell \the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}
      }{}
      }
	 \edef\n{\the\pgfmatrixcurrentrow} %the row
 	\edef\m{\the\pgfmatrixcurrentcolumn} %the column
	\edef\k{\the\numexpr\n+\quantikz@wires-1\relax}
	\settowidth{\myl}{g#2g}
	%if more than 1 wire, need to reserve space for each wire
	\ifnumequal{\quantikz@wires}{1}{}{
	 	\foreach \i in {\the\numexpr\n+1\relax,...,\k} {
 		%apply auto width to the cell, and make sure we unset the setting so that it doesn't apply to later circuits.
    \csxdef{cell@width@\i-\m}{\the\myl} %save the cell width for every row in a global variable
 	}
%		
 	}
	%\edef\n{\the\pgfmatrixcurrentrow}
	%\edef\m{\the\pgfmatrixcurrentcolumn}
	\expandafter\pgfutil@g@addto@macro\expandafter\tikzcd@atendsavedpaths\expandafter{%
		\expandafter\groupoutput@mid\expandafter{\newoptions}{#2}%
	}
}
%deferred labelling in the middle of circuits
\newcommand{\groupoutput@mid}[2]{%basic data as keys, label options, brace options, text
	\pgfkeys{/quantikz/gates/.cd,wires=1}
	\def\leftbrace{1}\def\rightbrace{1}
 	\pgfkeys{/quantikz/gates/.cd,#1}%
	\xdef\LoopGO{}
    \ifcsstringeitheror{wire@type@\quantikz@row}{c}{b}{%is the first wire classical? (should include bundle as well)
\xdef\LoopGO{\LoopGO($(\tikzcdmatrixname-\quantikz@row-\quantikz@col.center)+(0,\pgfkeysvalueof{/tikz/commutative diagrams/classical gap vertical})$)}
  }
   \ifcsstringeitheror{wire@type@\the\numexpr\quantikz@row+\quantikz@wires-1\relax}{c}{b}{%is the first wire classical? (should include bundle as well)
\xdef\LoopGO{\LoopGO($(\tikzcdmatrixname-\the\numexpr\quantikz@row+\quantikz@wires-1\relax-\quantikz@col.center)+(0,-\pgfkeysvalueof{/tikz/commutative diagrams/classical gap vertical})$)}
  }
	\foreach \n in  {\quantikz@row,...,\the\numexpr\quantikz@row+\quantikz@wires-1\relax} {
		\ifnodedefined{\tikzcdmatrixname-\n-\quantikz@col}{
			\xdef\LoopGO{\LoopGO(\tikzcdmatrixname-\n-\quantikz@col)} 
		}}
		\ifnumequal{\quantikz@wires}{1} {
		%\node (midgr-\row-\col) [fit=\LoopGO, inner sep=0pt,label={[align=center,#2]#4}] {};
		\node (midgr-\quantikz@row-\quantikz@col) [fit=\LoopGO, inner sep=0pt,label={[align=center,anchor=mid,expand style once=\quantikz@lstyle]center:#2}] {};
	}{
	\node (midgr-\quantikz@row-\quantikz@col) [fit=\LoopGO, inner sep=0pt,label={[align=center,anchor=mid,expand style once=\quantikz@lstyle]center:#2}] {};
	\ifthenelse{\rightbrace=1}{
	\draw[dm,expand style once=\quantikz@braces] ($(midgr-\quantikz@row-\quantikz@col.north east)+(-0.1cm,0.05cm)$) to ($(midgr-\quantikz@row-\quantikz@col.south east)+(-0.1cm,-0.05cm)$);
	}{}
	\ifthenelse{\leftbrace=1}{
	\draw[dd,expand style once=\quantikz@braces] ($(midgr-\quantikz@row-\quantikz@col.north west)+(0.1cm,0.05cm)$) to ($(midgr-\quantikz@row-\quantikz@col.south west)+(0.1cm,-0.05cm)$);
	}{}
	}
} %
%inputs and outputs within a multi-wire gate
\newcommand\gateinput[2][]{%
	\pgfkeys{/quantikz/gates/.cd,wires=1,style=,label style=,braces=,#1}%
	\edef\newoptions{row=\the\pgfmatrixcurrentrow,col=\the\pgfmatrixcurrentcolumn,#1}
   \ifnumless{\quantikz@wires}{0}{%
    \PackageError{quantikz}{You cannot have a gate input command with a negative number of wires. The culprit appears to be cell \the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}
    }{%
      \ifnumequal{\quantikz@wires}{0}{%
        \PackageError{quantikz}{You cannot have a gate input command with 0 wires. The culprit appears to be cell \the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}
      }{}
      }
	\expandafter\pgfutil@g@addto@macro\expandafter\tikzcd@atendlabels\expandafter{%
		\expandafter\mginput@end\expandafter{\newoptions}{#2}%
	}
}
\newcommand{\mginput@end}[2]{%collected options,label style, brace style,text
  \pgfkeys{/quantikz/gates/.cd,wires=1,label style=,braces=,style=,ps=,#1}%
%can we find the gategroup node?
\xdef\cell{group\tikzcdmatrixname-1-\quantikz@col}
\foreach \n in {\quantikz@row,...,1} {%
  %test if node group-\n-#2 exists
  \ifnodedefined{group\tikzcdmatrixname-\n-\quantikz@col}{%
      \xdef\cell{group\tikzcdmatrixname-\n-\quantikz@col}
      \breakforeach
  }{}
}
\ifnumequal{\quantikz@wires}{1}{%
  \node at ($(\cell.west |- \tikzcdmatrixname-\quantikz@row-\quantikz@col.west)+(0,0cm)$)[leftinternal,expand style once=\quantikz@lstyle]{#2};
}{%
%\show\quantwires
%\pgfmathsetmacro{\a}{\quantikz@row+\quantikz@wires-1}
\xdef\a{\tikzcdmatrixname-\the\numexpr\quantikz@row+\quantikz@wires-1\relax-\quantikz@col}
% \wlog{Quantikz intermediate output}
% \wlog{row: \quantikz@row}
% \wlog{wires: \quantikz@wires}
% \wlog{calculation:\a}
% \wlog{col: \quantikz@col}
% \wlog{matrix name: \tikzcdmatrixname}
\draw[dd,expand style once=\quantikz@braces] ($(\cell.west |- \tikzcdmatrixname-\quantikz@row-\quantikz@col.west)+(0.1cm,0.1cm)$) to node[leftinternal,midway,expand style once=\quantikz@lstyle] {#2} ($(\cell.west |- \a.west)+(0.1cm,-0.1cm)$);
}
} %
\newcommand\gateoutput[2][]{%
	\edef\newoptions{row=\the\pgfmatrixcurrentrow,col=\the\pgfmatrixcurrentcolumn,#1}
   \ifnumless{\quantikz@wires}{0}{%
    \PackageError{quantikz}{You cannot have a gate output command with a negative number of wires. The culprit appears to be cell \the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}
    }{%
      \ifnumequal{\quantikz@wires}{0}{%
        \PackageError{quantikz}{You cannot have a gate output command with 0 wires. The culprit appears to be cell \the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}
      }{}
      }
	\expandafter\pgfutil@g@addto@macro\expandafter\tikzcd@atendlabels\expandafter{%
		\expandafter\mgoutput@end\expandafter{\newoptions}{#2}%
	}
}
%deferred functions for the above
\newcommand{\mgoutput@end}[2]{%
	\pgfkeys{/quantikz/gates/.cd,wires=1,style=,label style=,braces=,#1}%
%can we find the gategroup node?
\xdef\cell{group\tikzcdmatrixname-1-\quantikz@col}
\foreach \n in {\quantikz@row,...,1} {%
	%test if node group-\n-#2 exists
	\ifnodedefined{group\tikzcdmatrixname-\n-\quantikz@col}{%
    	\xdef\cell{group\tikzcdmatrixname-\n-\quantikz@col}
    	\breakforeach
	}{}
}
\ifnumequal{\quantikz@wires}{1}{%
	\node at ($(\cell.east |- \tikzcdmatrixname-\quantikz@row-\quantikz@col.east)+(0,0cm)$)[rightinternal,expand style once=\quantikz@lstyle]{#2};
}{%
\xdef\a{\tikzcdmatrixname-\the\numexpr\quantikz@row+\quantikz@wires-1\relax-\quantikz@col}
\draw[dm,expand style once=\quantikz@braces] ($(\cell.east |- \tikzcdmatrixname-\quantikz@row-\quantikz@col.east)+(-0.1cm,0.1cm)$) to node[rightinternal,midway,expand style once=\quantikz@lstyle] {#2} ($(\cell.east |- \a.east)+(-0.1cm,-0.1cm)$);
}
} %

%wave command
\newcommand\wave[1][]{%
\setwiretype{n}
	\edef\n{\the\pgfmatrixcurrentrow}
	\expandafter\pgfutil@g@addto@macro\expandafter\tikzcd@atendslices\expandafter{%
		\expandafter\wave@end\expandafter{\n}{#1}%
	}
}
%deferred wave
\newcommand{\wave@end}[2]{
	\node (wave-#1) [fit=(\tikzcdmatrixname-row#1),wave,#2] {};
}


%put a border around a group of gates
\newcommand\gategroup[2][]{%
	\pgfkeys{/quantikz/gates/.cd,wires=1,style=,label style=,braces=,steps=1,#1}%
	\edef\newoptions{row=\the\pgfmatrixcurrentrow,col=\the\pgfmatrixcurrentcolumn,#1}
   \ifnumless{\quantikz@wires}{0}{%
    \PackageError{quantikz}{You cannot have a gate group command with a negative number of wires. The culprit appears to be cell \the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}
    }{%
      \ifnumequal{\quantikz@wires}{0}{%
        \PackageError{quantikz}{You cannot have a gate group command with 0 wires. The culprit appears to be cell \the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}
      }{}
      }
   \ifnumless{\quantikz@steps}{0}{%
    \PackageError{quantikz}{You cannot have a gate group command with a negative number of steps. The culprit appears to be cell \the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}
    }{%
      \ifnumequal{\quantikz@steps}{0}{%
        \PackageError{quantikz}{You cannot have a gate group command with 0 steps. The culprit appears to be cell \the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}
      }{}
      }
	\expandafter\pgfutil@g@addto@macro\expandafter\tikzcd@atendlabels\expandafter{%
		\expandafter\gategroup@end\expandafter{\newoptions}{#2}%
	}
}
%deferred gate group command
\newcommand{\gategroup@end}[2]{%options, gate style, text style, text
	\pgfkeys{/quantikz/gates/.cd,wires=1,style=,label style=,braces=,steps=1}%
	\edef\background{0}%
	\pgfkeys{/quantikz/gates/.cd,#1}%
	\edef\fit{(\tikzcdmatrixname-col\quantikz@col.west |- \tikzcdmatrixname-row\quantikz@row.north)(\tikzcdmatrixname-col\the\numexpr\quantikz@col+\quantikz@steps-1\relax.east |- \tikzcdmatrixname-row\the\numexpr\quantikz@row+\quantikz@wires-1\relax.south)}%
	\ifthenelse{\background=1}{%
		\begin{pgfonlayer}{background}\node (ggroup-\quantikz@row-\quantikz@col) [fit=\fit,ggroup,label={[group label,expand style once=\quantikz@lstyle]:#2},expand style once=\quantikz@style] {};\end{pgfonlayer}
	}{%
		\node (ggroup-\quantikz@row-\quantikz@col) [fit=\fit,ggroup,label={[group label,expand style once=\quantikz@lstyle]:#2},expand style once=\quantikz@style] {};
	}
}


%this command runs after we've finished the matrix, and makes unified cells for each row and each column. This allows much nicer alignment of large boxes.
\newcommand{\DivideRowsCols}{
	\foreach \n in {1,...,\the\pgfmatrixcurrentrow} {%for each row, construct a master cell that contains all entries
	\xdef\LoopRow{}
		\foreach \m in {1,...,\the\pgfmatrixcurrentcolumn}{
			\ifnodedefined{\tikzcdmatrixname-\n-\m}{
				\xdef\LoopRow{\LoopRow(\tikzcdmatrixname-\n-\m)}
			}{}
			\ifnodedefined{group\tikzcdmatrixname-\n-\m}{
				\xdef\LoopRow{\LoopRow(group\tikzcdmatrixname-\n-\m)}
			}{}
	}
	\node (\tikzcdmatrixname-row\n) [fit=\LoopRow] {};
	}
	\foreach \n in {1,...,\the\pgfmatrixcurrentcolumn} {%for each column, construct a master cell that contains all entries
	\xdef\LoopCol{}
		\foreach \m in {1,...,\the\pgfmatrixcurrentrow}{
			\ifnodedefined{\tikzcdmatrixname-\m-\n}{
				\xdef\LoopCol{\LoopCol(\tikzcdmatrixname-\m-\n)}
			}{}
			\ifnodedefined{group\tikzcdmatrixname-\m-\n}{
				\xdef\LoopCol{\LoopCol(group\tikzcdmatrixname-\m-\n)}
			}{}
	}
	\node (\tikzcdmatrixname-col\n) [fit=\LoopCol] {};
	}
}

%this is the command that implements the align equals at key.
%take a parameter, row number, where we want to set the baseline. if not integer, use the two rows spanned
\providecommand{\setmiddle}[1]{%
\IfInteger{#1}{
\pgfmathtruncatemacro\wholepart{floor(#1)}
\edef\temp{\noexpand\tikzset{%
/tikz/baseline={([yshift=-\MathAxis]\noexpand\tikzcdmatrixname-\wholepart-1.center)}
}}
%\show\temp
\temp
}{%
\pgfmathtruncatemacro\wholepart{floor(#1)}
\pgfmathtruncatemacro\neighbour{floor(#1)+1}
\pgfmathsetmacro\fractionalpart{#1-floor(#1)}
\edef\temp{
%\noexpand\tikzset{every matrix/.append style={baseline=([yshift=-\MathAxis]$(\noexpand\tikzcdmatrixname-\wholepart-1.base)!\fractionalpart!(\noexpand\tikzcdmatrixname-\neighbour-1.base)$)}%
\noexpand\tikzset{%
/tikz/baseline={([yshift=-\MathAxis]$(\noexpand\tikzcdmatrixname-\wholepart-1.center)!\fractionalpart!(\noexpand\tikzcdmatrixname-\neighbour-1.center)$)}
}}
%\show\temp
\temp
}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Option parameter processing via key/value pairs
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\tikzcdset{
  row sep/normal=0.5cm,
  column sep/normal=0.5cm,
  }
%initialise all the pgfkeys for key=value parameter passing in macro options
\tikzcdset{%
	slice all/.code={\gdef\toslice@qtkz{1}},
	remove end slices/.initial=0,
	slice titles/.initial={\col},
	slice style/.initial={},
	slice label style/.initial={},
	thin lines/.code={\resetstyles},
	transparent/.code={\maketransparent},
	vertical slice labels/.code={\def\vert@qtkz{1}},
	align equals at/.code={\setmiddle{#1}},
  wire types/.code={\importwiretypes{#1}},
  classical gap horizontal/.initial=0.03cm, % define separation of classical wires (can override)
  classical gap vertical/.initial=0.03cm, % define separation of classical wires (can override)
  classical gap/.code={
    \tikzcdset{classical gap horizontal={#1},classical gap vertical={#1}}
  },
 % wire style/.code={\gdef\quantikzopts{#1}},
}
\pgfkeys{/quantikz/gates/.cd,%
	.unknown/.style={%
		/quantikz/gates/wires=\pgfkeyscurrentname
	},%
	%wires/.store in=\quantwires,%
	%wires/.initial=1,%
	%style/.initial={},
	%label style/.initial={},
	%braces/.initial={},
	background/.code={\def\background{1}},
	%alternate/.default=1,
	%alternate/.code={\def\helper{#1}},
  alternate/.code={\PackageWarning{quantikz}{Use of alternate is deprecated.}},
	%row/.initial=1,
	%col/.initial=1,
	%steps/.initial=1,
	%Strike Width/.initial=0.08cm,
	%Strike Height/.initial=0.12cm,
	swap/.code={\def\toswap{1}},
	disable auto height/.code={\def\DisableMinSize{1}},
  nwires/.code={\PackageWarning{quantikz}{Use of nwires is deprecated. Set wire types globally instead.}},
  cwires/.code={\PackageWarning{quantikz}{Use of cwires is deprecated. Set wire types globally instead.}},
	brackets/.is choice,
	brackets/.initial=both,
  %priority label/.initial={},
  ps/.initial={},
  %angle/.initial=-45,
  %vertical wire/.initial=q,
  %wire style/.initial={},
  open/.code={\tikzset{filling}},
  %partial swap/.initial={},
  %partial position/.initial={0.5},
}
\pgfkeys{/quantikz/gates/brackets/.cd,%define brackets options
	none/.code={\def\leftbrace{0}\def\rightbrace{0}},
	left/.code={\def\leftbrace{1}\def\rightbrace{0}},
	right/.code={\def\leftbrace{0}\def\rightbrace{1}},
	both/.code={\def\leftbrace{1}\def\rightbrace{1}}
}
% \pgfkeys{/quantikz/swap/.cd,%define options for swap gate
%   partial/.initial={},
%   position/.initial={0.5},
%   label style/.initial={}
% }


%my standard Dirac notation commands. can be overridden by user.
\providecommand{\ket}[1]{\ensuremath{\left|#1\right\rangle}}
\providecommand{\bra}[1]{\ensuremath{\left\langle#1\right |}}
\providecommand{\proj}[1]{\ensuremath{\ket{#1}\!\bra{#1}}}
\providecommand{\braket}[2]{\ensuremath{\left\langle#1\middle|#2\right\rangle}}
\newcommand{\forceredefine}{%
\renewcommand{\ket}[1]{\ensuremath{\left|##1\right\rangle}}
\renewcommand{\bra}[1]{\ensuremath{\left\langle##1\right |}}
\renewcommand{\proj}[1]{\ensuremath{\ket{##1}\!\bra{##1}}}
\renewcommand{\braket}[2]{\ensuremath{\left\langle##1\middle|##2\right\rangle}}
}


%\DeclareExpandableDocumentCommand{\ctrlbundle}{O{1}O{}m}{|[phase bundle,#2]| {} \vqw{#3}\qwbundle[alternate=#1]{}}

%wire commands with absolute positioning. Need updating.
\newcommand{\vqwexplicit}[2]{
	\arrow[from=#1,to=#2,arrowStyle] {}
}
% \newcommand{\vqbundleexplicit}[2]{
% 	\arrow[from=#1,to=#2,arrows] {} \arrow[from=#1,to=#2,arrows,yshift=0.1cm] {}\arrow[from=#1,to=#2,arrows,yshift=-0.1cm] {}
% }
% %classical vertical wire, absolute positioning
% \newcommand{\vcwexplicit}[2]{
% 	\arrow[from=#1,to=#2,arrows,xshift=0.05cm] {}\arrow[from=#1,to=#2,arrows,xshift=-0.05cm] {}
% }
% %classical horizontal wire, absolute positioning
% \newcommand{\vcwhexplicit}[2]{
% 	\arrow[from=#1,to=#2,arrows,yshift=0.05cm] {}\arrow[from=#1,to=#2,arrows,yshift=-0.05cm] {}
% }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Style properties
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%configure some of the style properties.
%annoyingly, this first one will affect all tikzcd instances, not just quantum circuits. I should have only provided the quantikz environment as a modified version of tikzcd, and not allowed direct use of tikzcd. Probably too late now.

\tikzset{
	thickness/.style={thick},
  filling/.style={fill=\pgfkeysvalueof{/tikz/commutative diagrams/background color}},
  operator/.style={draw,filling, inner sep=2pt,thickness,align=center},
  ggroup/.style={draw,minimum size=1.5em,thickness,align=center,inner sep=4pt},
  leftinternal/.style={anchor=mid west,font=\scriptsize,inner sep=4pt,align=center},
  rightinternal/.style={anchor=mid east,font=\scriptsize,inner sep=4pt,align=center},
  wave/.style={inner sep=-3pt,tape,filling,apply={draw=black} except on segments {5,6,1,2,9}},
  phase bundle/.style={fill,shape=rectangle,rounded corners=1.5pt,minimum width=4pt,minimum height=10pt},
  internal/.style={thickness},
 %  rectangle with rounded corners north west/.initial=0pt,
	% rectangle with rounded corners south west/.initial=0pt,
	% rectangle with rounded corners north east/.initial=8pt,
	% rectangle with rounded corners south east/.initial=8pt,
  line/.style={path picture={ 
		\draw[internal](path picture bounding box.west) -- (path picture bounding box.east);
	}},
	%hidden bend/.style={path picture={
%		\draw[internal,inner sep=0pt] (path picture bounding box.west) -- (path picture bounding box.center) -- (path picture bounding box.south);},
%		minimum height=1.5em,minimum width=1em},
  dd/.style={decoration={brace},decorate,thickness},
  dm/.style={decoration={brace,mirror},decorate,thickness},
  slice/.style={thickness,red,dash pattern=on 5pt off 3pt,align=center},
 	my labelcw/.style={yshift=0.04cm,above,align=center},
 	gg label/.style={label position=center,align=center},
 	group label/.style={label position=above,yshift=0.2cm,anchor=mid}
}

\def\resetstyles{
\tikzcdset{thin,every cell/.append style={thin},arrowStyle/.append style={thin}
    }
\tikzset{
	thickness/.style={thin},
	%operator/.append style={thin},
	%internal/.append style={thin},
	%dd/.append style={thin},
	%dm/.append style={thin},
	%slice/.append style={thin},
	meter/.append style={thin},
	phase/.append style={minimum size=3pt},
%	ophase/.append style={minimum size=3pt},
	%circlewc/.append style={minimum size=3pt,inner sep=2pt}
}
}

\def\maketransparent{
\tikzset{
  filling/.append style={fill opacity=0,text opacity=1},
%	operator/.append style={fill opacity=0},
	% meter/.append style={fill opacity=0},
	% measuretab/.append style={fill opacity=0},
	% meterD/.append style={fill opacity=0},
	% measure/.append style={fill opacity=0},
	% wave/.append style={fill opacity=0},
%	ophase/.append style={fill opacity=0}
}
}

